"I need a better description'': An Investigation Into User Expectations For Differential Privacy

Despite recent widespread deployment of differential privacy, relatively little is known about what users think of differential privacy. In this work, we seek to explore users' privacy expectations related to differential privacy. Specifically, we investigate (1) whether users care about the protections afforded by differential privacy, and (2) whether they are therefore more willing to share their data with differentially private systems. Further, we attempt to understand (3) users' privacy expectations of the differentially private systems they may encounter in practice and (4) their willingness to share data in such systems. To answer these questions, we use a series of rigorously conducted surveys (n=2424). We find that users care about the kinds of information leaks against which differential privacy protects and are more willing to share their private information when the risks of these leaks are less likely to happen. Additionally, we find that the ways in which differential privacy is described in-the-wild haphazardly set users' privacy expectations, which can be misleading depending on the deployment. We synthesize our results into a framework for understanding a user's willingness to share information with differentially private systems, which takes into account the interaction between the user's prior privacy concerns and how differential privacy is described.

==> methods.tex <==
\section{Methods}\label{sec:methods}
We now give an overview of our survey methodology.  Our full survey instruments can be found in \cref{apx:surveys}. Our procedures were approved by our institution's ethics review board.

To answer our research questions, we ran two surveys ($n = 2424$ total), one to address RQ1 and RQ2 and the other to address RQ3 and RQ4. In order to improve the external validity of our work, we use vignette (scenario) surveys~\cite{hainmueller2015validating}. In both our surveys, we use the same two scenarios, which focus on two different potential use cases for DP: protecting people's salaries and protecting people's medical histories. To contextualize the first scenario, we ask respondents to imagine that they work in the banking industry and are approached by a friend on behalf of a salary transparency initiative. In the second scenario, we ask the respondent to imagine that during their next doctor's visit, their doctor asks them if they want to share their medical records with a medical research non-profit, in the name of improving care. The exact wording of these scenarios is shown in \cref{tab:scenariosandexpectation}. We ran both surveys using Amazon Mechanical Turk (MTurk).  MTurk has been shown to be representative of American privacy preferences for Americans aged 18-50 who have at least some college education~\cite{SP:RedKroMaz19}.


% \input{branch34}

% \input{branch12}

\subsection{Limitations}
As in all user studies, our study is subject to multiple possible biases. The first is sampling bias. We sample our respondents using MTurk. While prior work shows that MTurk is reasonably representative of the privacy attitudes and experiences of Americans aged 18-50 who have some college education ~\cite{SP:RedKroMaz19}, our sample does not capture the experiences of all Americans, especially those older and less educated. Our results should be interpreted in this context.  Second, we may have introduced reporting biases through our question design. While we aimed to follow best practices --- using cognitive interviews to validate our questionnaire, and offering ``other'' and ``I don't know'' response options~\cite{redmiles2017summary} --- respondents may still have mis-reported or failed to report their true perceptions or preferences. Third, while we took steps to improve external validity --- sourcing experimental stimuli by rigorously collecting and coalescing in-the-wild DP descriptions and using a vignette survey --- our study may have failed to appropriately reflect real-world conditions.

==> padjust.tex <==
\begin{table*}[h!t]
\centering
\small
\begin{tabular}{lcr|cr|cr|cr|cr|cr} 
 \toprule
 \multicolumn{1}{c}{\textbf{Variable}} & \multicolumn{2}{|c}{\textbf{\emph{Hack}}} & \multicolumn{2}{|c}{\textbf{\emph{Law Enforcement}}} & \multicolumn{2}{|c}{\textbf{\emph{\exactexpectationname}}} & \multicolumn{2}{|c}{\textbf{\emph{Data Analyst}}} & \multicolumn{2}{|c}{\textbf{\emph{Graphs}}} & \multicolumn{2}{|c}{\textbf{\emph{Share}}}\\
 \midrule
  & OR/CI & p-value & OR/CI & p-value & OR/CI & p-value & OR/CI & p-value & OR/CI & p-value & OR/CI & p-value \\ 
 \midrule
 Description: & \textbf{1.94} & \multirow{2}{*}{\textbf{0.01*}} & 1.10 & \multirow{2}{*}{0.72} & 1.13 & \multirow{2}{*}{0.59} & 1.71 & \multirow{2}{*}{0.1} & \textbf{1.64} & \multirow{2}{*}{\textbf{0.05*}} & 1.68 & \multirow{2}{*}{0.06} \\ 
~~ \emph{Unsubstantial} & {\scriptsize [1.16, 3.29]} & & {\scriptsize [0.65, 1.86]} & & {\scriptsize [0.73, 1.75]} & & {\scriptsize [0.92, 3.27]} & & {\scriptsize [1.01, 2.67]} & & {\scriptsize [0.99, 2.88]} & \\
Description: & \textbf{1.96} & \multirow{2}{*}{\textbf{0.01*}} & 1.21 & \multirow{2}{*}{0.47} & 1.43 & \multirow{2}{*}{0.1} & \textbf{2.40} & \multirow{2}{*}{\textbf{$<$ 0.01**}} & \textbf{2.15} & \multirow{2}{*}{\textbf{$<$ 0.01**}} & \textbf{2.22} & \multirow{2}{*}{\textbf{$<$ 0.01**}} \\ 
~~ \emph{Techniques} & {\scriptsize [1.17, 3.33]} & & {\scriptsize [0.72, 2.03]} & & {\scriptsize [0.93, 2.22]} & & {\scriptsize [1.33, 4.5]} & & {\scriptsize [1.34, 3.5]} & & {\scriptsize [1.33, 3.77]} & \\
Description: & 1.60 & \multirow{2}{*}{0.08} & 1.05 & \multirow{2}{*}{0.84} & 1.40 & \multirow{2}{*}{0.13} & \textbf{2.06} & \multirow{2}{*}{\textbf{0.02*}} & \textbf{1.76} & \multirow{2}{*}{\textbf{0.02*}} & 1.69 & \multirow{2}{*}{0.05} \\ 
~~ \emph{Enables} & {\scriptsize [0.95, 2.73]} & & {\scriptsize [0.63, 1.77]} & & {\scriptsize [0.91, 2.16]} & & {\scriptsize [1.13, 3.88]} & & {\scriptsize [1.09, 2.87]} & & {\scriptsize [1, 2.9]} & \\
Description: & \textbf{1.86} & \multirow{2}{*}{\textbf{0.02*}} & 1.04 & \multirow{2}{*}{0.89} & 1.43 & \multirow{2}{*}{0.11} & \textbf{1.99} & \multirow{2}{*}{\textbf{0.03*}} & 1.38 & \multirow{2}{*}{0.2} & 1.19 & \multirow{2}{*}{0.55} \\ 
~~ \emph{Trust} & {\scriptsize [1.11, 3.17]} & & {\scriptsize [0.61, 1.76]} & & {\scriptsize [0.92, 2.22]} & & {\scriptsize [1.08, 3.78]} & & {\scriptsize [0.84, 2.28]} & & {\scriptsize [0.68, 2.09]} & \\
Description: & \textbf{2.58} & \multirow{2}{*}{\textbf{$<$ 0.01***}} & \textbf{1.86} & \multirow{2}{*}{\textbf{0.01*}} & 1.43 & \multirow{2}{*}{0.1} & \textbf{2.46} & \multirow{2}{*}{\textbf{$<$ 0.01**}} & \textbf{2.40} & \multirow{2}{*}{\textbf{$<$ 0.01***}} & \textbf{2.27} & \multirow{2}{*}{\textbf{$<$ 0.01**}} \\ 
~~\emph{Risk} & {\scriptsize [1.57, 4.33]} & & {\scriptsize [1.15, 3.05]} & & {\scriptsize [0.93, 2.2]} & & {\scriptsize [1.37, 4.59]} & & {\scriptsize [1.5, 3.88]} & & {\scriptsize [1.37, 3.84]} & \\
Description: & 1.56 & \multirow{2}{*}{0.1} & 1.02 & \multirow{2}{*}{0.95} & 1.38 & \multirow{2}{*}{0.15} & \textbf{2.30} & \multirow{2}{*}{\textbf{0.01**}} & \textbf{1.70} & \multirow{2}{*}{\textbf{0.03*}} & \textbf{1.90} & \multirow{2}{*}{\textbf{0.02*}} \\ 
~~\emph{Technical} & {\scriptsize [0.92, 2.69]} & & {\scriptsize [0.6, 1.73]} & & {\scriptsize [0.89, 2.14]} & & {\scriptsize [1.26, 4.33]} & & {\scriptsize [1.04, 2.79]} & & {\scriptsize [1.12, 3.25]} & \\
\midrule
\multirow{2}{*}{Salary Scenario} & \textbf{1.32} & \multirow{2}{*}{\textbf{0.04*}} & 0.80 & \multirow{2}{*}{0.11} & \textbf{1.29} & \multirow{2}{*}{\textbf{0.03*}} & 0.75 & \multirow{2}{*}{0.06} & 1.23 & \multirow{2}{*}{0.1} & 1.14 & \multirow{2}{*}{0.31} \\ 
& {\scriptsize [1.02, 1.71]} & & {\scriptsize [0.61, 1.05]} & & {\scriptsize [1.03, 1.63]} & & {\scriptsize [0.56, 1.01]} & & {\scriptsize [0.96, 1.57]} & & {\scriptsize [0.88, 1.49]} & \\
\multirow{2}{*}{Internet Score} & \textbf{1.17} & \multirow{2}{*}{\textbf{0.04*}} & \textbf{1.25} & \multirow{2}{*}{\textbf{0.01**}} & 1.02 & \multirow{2}{*}{0.78} & 1.05 & \multirow{2}{*}{0.54} & 1.07 & \multirow{2}{*}{0.36} & 1.01 & \multirow{2}{*}{0.85} \\ 
& {\scriptsize [1.01, 1.36]} & & {\scriptsize [1.06, 1.46]} & & {\scriptsize [0.89, 1.17]} & & {\scriptsize [0.89, 1.25]} & & {\scriptsize [0.93, 1.23]} & & {\scriptsize [0.87, 1.18]} & \\
 
  \bottomrule
\end{tabular}
\caption{\small \label{tab:betterbydefn} Logistic regression models of the relationship between the DP description a respondent was shown and their perception of the likelihood that their information will be disclosed through a particular information flow. See Table~\ref{tab:explicityexpectationssharing} for detailed legend.}
\end{table*}

==> results.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.48\textwidth]{figures/prop_care_expectation.pdf}
  %\vspace{-3ex}
  \caption{\small Proportion of respondents who care about each potential information disclosure.}
  \label{fig:propcare}
  \vspace{-3ex}
%   \vspace{-1em}
\end{figure}

\begin{table*}[h!t]
\centering
\small


\begin{tabular}{lcr|cr|cr|cr|cr|cr} 
 \toprule
 \multicolumn{1}{c|}{\textbf{Variable}} & \multicolumn{2}{c|}{\textbf{\emph{Hack}}} & \multicolumn{2}{c|}{\textbf{\emph{Law Enforcement}}} & \multicolumn{2}{c|}{\textbf{\emph{\exactexpectationname}}} & \multicolumn{2}{c|}{\textbf{\emph{Data Analyst}}} & \multicolumn{2}{c|}{\textbf{\emph{Graphs}}} & \multicolumn{2}{c}{\textbf{\emph{Share}}}\\
 \midrule
  & OR/CI & p-value & OR/CI & p-value & OR/CI & p-value & OR/CI & p-value & OR/CI & p-value & OR/CI & p-value \\ 

 \midrule
 \multirow{2}{*}{Low Risk} & \textbf{1.91} & \multirow{2}{*}{\textbf{$<$ 0.01**}} & 0.87 & \multirow{2}{*}{0.55} & \textbf{1.63} & \multirow{2}{*}{\textbf{ 0.01*}} & 0.92 & \multirow{2}{*}{0.72} & 1.42 & \multirow{2}{*}{ 0.14} & 1.25 & \multirow{2}{*}{ 0.27} \\ 
& {\scriptsize [1.27, 2.88]}& & {\scriptsize [0.54, 1.39]}& & {\scriptsize [1.12, 2.38]}& & {\scriptsize [0.59, 1.44]}& & {\scriptsize [0.89, 2.27]}& & {\scriptsize [0.85, 1.84]} & \\
\multirow{2}{*}{No Risk} & \textbf{2.97} & \multirow{2}{*}{\textbf{$<$ 0.01***}} & \textbf{2.07} & \multirow{2}{*}{ \textbf{$<$ 0.01**}} & \textbf{1.61} & \multirow{2}{*}{\textbf{0.01*}} & 1.23 & \multirow{2}{*}{0.36} & 1.48 & \multirow{2}{*}{0.1} & \textbf{1.97} & \multirow{2}{*}{\textbf{$<$ 0.01***}} \\

& {\scriptsize [1.98, 4.49]}& & {\scriptsize [1.32, 3.27]}& & {\scriptsize [1.1, 2.35]}& & {\scriptsize [0.79, 1.9]}& & {\scriptsize [0.93, 2.37]}& & {\scriptsize [1.35, 2.88]} & \\
\midrule
\multirow{2}{*}{Salary Scenario} & \textbf{1.44} & \multirow{2}{*}{\textbf{0.03*}} & 1.35 & \multirow{2}{*}{0.12} & 1.20 & \multirow{2}{*}{0.23} & 1.37 & \multirow{2}{*}{0.09} & 1.12 & \multirow{2}{*}{0.54} & 1.04 & \multirow{2}{*}{0.81} \\ 
& {\scriptsize [1.04, 2]}& & {\scriptsize [0.92, 1.98]}& & {\scriptsize [0.89, 1.64]}& & {\scriptsize [0.96, 1.96]}& & {\scriptsize [0.77, 1.64]}& & {\scriptsize [0.76, 1.42]} & \\
\multirow{2}{*}{Internet Score} & 1.04 & \multirow{2}{*}{ 0.68} & 1.01 & \multirow{2}{*}{ 0.92} &0.98 & \multirow{2}{*}{ 0.79} & \textbf{1.24} & \multirow{2}{*}{\textbf{ 0.04*}} & 1.05 & \multirow{2}{*}{ 0.66} & 1.01 & \multirow{2}{*}{0.87} \\ 
& {\scriptsize [0.86, 1.25]} & & {\scriptsize [0.82, 1.24]} & & {\scriptsize [0.82, 1.16]} & & {\scriptsize [1.01, 1.52]} & & {\scriptsize [0.86, 1.28]} & & {\scriptsize [0.86, 1.2]} & \\

  \bottomrule
\end{tabular}
\caption{\small \label{tab:explicityexpectationssharing} Effect of expectation about the probability of a disclosure on respondent willingness to share. Each logistic regression model constructed only for respondents who cared about that type of disclosure, comparing against the High Risk condition. Table shows odds ratio (OR), 95\% confidence intervals for the odds ratios (shown in brackets), and p-values, where * indicates $p<0.05$, ** indicates $p<0.01$, and *** indicates $p<0.001$.}
\vspace{-2em}
\end{table*}

\section{Results}\label{sec:results}
% \clearpage
%\subsection{Does Knowing That Data Is Protected By DP Increase Likelihood of Sharing?}
Here, we detail the results of our analyses addressing RQ1-4.

\subsection{RQ1: What Information Disclosures Concern Users?} \label{sec:cares}
The goal of DP is to protect user information against disclosure to various entities. Thus, we  investigate whether users care about potential information disclosures to different entities against which DP can protect (see Table~\ref{tab:scenariosandexpectation} for information disclosures and  Section~\ref{sec:surveyone} the source of these disclosures).
 
We find that the most respondents --- 60.3\% --- care information disclosures to third-parties (Share). Over half (55.3\%) care about disclosures to the person or organization running the initiative to which they contributed their information, while 52.1\% care about disclosure of their information to an entity that hacks the organization to which they contributed their information. Fewer, 43.5\%, care about whether a data analyst working at the organization might be able to learn their private information or whether graphs created using their information might disclose their private information (40.8\%). Finally, 39.8\% of respondents care whether law enforcement might be able to access their information using a court order.% See \cref{fig:propcare}.

It is interesting to note that nearly 20\% more respondents ($\chi^2=34.54$, $p<0.001$) cared about their information being disclosed to a third party vs. being disclosed through graphs created using their information. Similarly, 11.8\% more respondents ($\chi^2=22.32$, $p<0.001$) cared about their information being disclosed to the organization running the initiative vs. being disclosed specifically to a data analyst at the organization. Open-answer responses offer some insight into this difference. When asked why they would (or would not) be willing to share their information, after they were told the risk of the disclosures they indicated they cared about, many respondents indicated that they believed in the cause of the initiative and wanted to contribute to their analysis/research. For example, one respondent said ``I trust the non-profit organization to handle my information responsibly and to use it for the positive research purpose that they claim they will be using it for.'' Thus, respondents may care less about disclosures that occur through ``appropriate information flows''~\cite{nissenbaum2004privacy}, in which user's information is being used in the way they expect: to benefit e.g., salary transparency or medical research through data analysis and the generation of graphs.% However, they may still be concerned about their data leaking to a person or organization that may be using their data in other ways.

\begin{table*}[h!t]
\centering
\small
\begin{tabular}{lcr|cr|cr|cr|cr|cr} 
 \toprule
 \multicolumn{1}{c}{\textbf{Variable}} & \multicolumn{2}{|c}{\textbf{\emph{Hack}}} & \multicolumn{2}{|c}{\textbf{\emph{Law Enforcement}}} & \multicolumn{2}{|c}{\textbf{\emph{\exactexpectationname}}} & \multicolumn{2}{|c}{\textbf{\emph{Data Analyst}}} & \multicolumn{2}{|c}{\textbf{\emph{Graphs}}} & \multicolumn{2}{|c}{\textbf{\emph{Share}}}\\
 \midrule
  & OR/CI & p-value & OR/CI & p-value & OR/CI & p-value & OR/CI & p-value & OR/CI & p-value & OR/CI & p-value \\ 
 \midrule
%  Description: \emph{Unsubstantial}	&		 1.13 &			 0.59 & \textbf{1.94} &	 \textbf{0.01*} & 1.10 &	 0.72 & 1.71 &	 0.1 & \textbf{1.64} &	 \textbf{0.05*} & 1.68 &	 0.06 \\ 
%  Description: \emph{Techniques}	&		 1.43 &			 0.1 & \textbf{1.96} &	 \textbf{0.01*} & 1.21 &	 0.47 & \textbf{2.40} &	 $<$ \textbf{0.01**} & 2.15 &	 $<$ \textbf{0.01**} & 2.22 &	 $<$ \textbf{0.01**} \\ 
% Description: \emph{Enables} 		&		 1.40 &			 0.13 & 1.60 &	 0.08 & 1.05 &	 0.84 & \textbf{2.06} &	 \textbf{0.02*} & \textbf{1.76} &	 \textbf{0.02*} & 1.69 &	.05 \\ 
%  Description: \emph{Trust} 		&	 1.43 &			 0.11 & \textbf{1.86} & \textbf{0.02*} & 1.04 &	 0.89 & \textbf{1.99} &	 \textbf{0.03}* & 1.38 &	 0.2 & 1.19 &	 0.55 \\ 
% Description: \emph{Risk} 			&	 1.43 &			 0.1 & \textbf{2.58} &	 $<$ \textbf{0.01***} & \textbf{1.86} &	 \textbf{0.01*} & \textbf{2.46} &	 $<$ \textbf{0.01**} & \textbf{2.40} &	 $<$ \textbf{0.01***} & \textbf{2.27} &	 $<$ \textbf{0.01**} \\ 
% Description: \emph{Technical} 		&		 1.38 &			 0.15 & 1.56 &	 0.1 & 1.02 &	 0.95 & \textbf{2.30} &	 \textbf{0.01**} & \textbf{1.70} &	 \textbf{0.03*} & \textbf{1.90} &	 \textbf{0.02*} \\ 
% \midrule
% Salary Scenario &	\textbf{1.29} &	 \textbf{0.03*} & \textbf{1.32} &	 \textbf{0.04*} & 0.80 &	 0.11 & 0.75 &	 0.06 & 1.23 &	 0.1 & 1.14 &	0.31 \\ 
% Internet Score &			 1.02 &			 0.78 & \textbf{1.17} &	 \textbf{0.04*} & \textbf{1.25} &	 \textbf{0.01**} & 1.05 &	 0.54 & 1.07 &	 0.36 & 1.01 &	 0.85 \\ 

% \midrule

% Description: & 1.13 & \multirow{2}{*}{0.59} & \textbf{1.94} & \multirow{2}{*}{\textbf{0.01*}} & 1.10 & \multirow{2}{*}{0.72} & 1.71 & \multirow{2}{*}{0.1} & \textbf{1.64} & \multirow{2}{*}{\textbf{0.05*}} & 1.68 & \multirow{2}{*}{0.06} \\ 
% ~~ \emph{Unsubstantial}& {\scriptsize [0.73, 1.75]} & & {\scriptsize [1.16, 3.29]} & & {\scriptsize [0.65, 1.86]} & & {\scriptsize [0.92, 3.27]} & & {\scriptsize [1.01, 2.67]} & & {\scriptsize [0.99, 2.88]} & \\
% Description: & 1.43 & \multirow{2}{*}{0.1} & \textbf{1.96} & \multirow{2}{*}{\textbf{0.01*}} & 1.21 & \multirow{2}{*}{0.47} & \textbf{2.40} & \multirow{2}{*}{\textbf{$<$ 0.01**}} & \textbf{2.15} & \multirow{2}{*}{\textbf{$<$ 0.01**}} & \textbf{2.22} & \multirow{2}{*}{\textbf{$<$ 0.01**}} \\ 
% ~~ \emph{Techniques}& {\scriptsize [0.93, 2.22]} & & {\scriptsize [1.17, 3.33]} & & {\scriptsize [0.72, 2.03]} & & {\scriptsize [1.33, 4.5]} & & {\scriptsize [1.34, 3.5]} & & {\scriptsize [1.33, 3.77]} & \\
% Description: & 1.40 & \multirow{2}{*}{0.13} & 1.60 & \multirow{2}{*}{0.08} & 1.05 & \multirow{2}{*}{0.84} & \textbf{2.06} & \multirow{2}{*}{\textbf{0.02*}} & \textbf{1.76} & \multirow{2}{*}{\textbf{0.02*}} & 1.69 & \multirow{2}{*}{0.05} \\ 
% ~~ \emph{Enables}& {\scriptsize [0.91, 2.16]} & & {\scriptsize [0.95, 2.73]} & & {\scriptsize [0.63, 1.77]} & & {\scriptsize [1.13, 3.88]} & & {\scriptsize [1.09, 2.87]} & & {\scriptsize [1, 2.9]} & \\
% Description: & 1.43 & \multirow{2}{*}{0.11} & \textbf{1.86} & \multirow{2}{*}{\textbf{0.02*}} & 1.04 & \multirow{2}{*}{0.89} & 1.99 & \multirow{2}{*}{\textbf{0.03*}} & 1.38 & \multirow{2}{*}{0.2} & 1.19 & \multirow{2}{*}{0.55} \\ 
% ~~ \emph{Trust} & {\scriptsize [0.92, 2.22]} & & {\scriptsize [1.11, 3.17]} & & {\scriptsize [0.61, 1.76]} & & {\scriptsize [1.08, 3.78]} & & {\scriptsize [0.84, 2.28]} & & {\scriptsize [0.68, 2.09]} & \\
% Description: & 1.43 & \multirow{2}{*}{0.1} & \textbf{2.58} & \multirow{2}{*}{\textbf{$<$ 0.01***}} & \textbf{1.86} & \multirow{2}{*}{\textbf{0.01*}} & \textbf{2.46} & \multirow{2}{*}{\textbf{$<$ 0.01**}} & \textbf{2.40} & \multirow{2}{*}{\textbf{$<$ 0.01***}} & \textbf{2.27} & \multirow{2}{*}{\textbf{$<$ 0.01**}} \\ 
% ~~\emph{Risk} & {\scriptsize [0.93, 2.2]} & & {\scriptsize [1.57, 4.33]} & & {\scriptsize [1.15, 3.05]} & & {\scriptsize [1.37, 4.59]} & & {\scriptsize [1.5, 3.88]} & & {\scriptsize [1.37, 3.84]} & \\
% Description: & 1.38 & \multirow{2}{*}{0.15} & 1.56 & \multirow{2}{*}{0.1} & 1.02 & \multirow{2}{*}{0.95} & \textbf{2.30} & \multirow{2}{*}{\textbf{0.01**}} & \textbf{1.70} & \multirow{2}{*}{\textbf{0.03*}} & \textbf{1.90} & \multirow{2}{*}{\textbf{0.02*}} \\ 
% ~~\emph{Technical} & {\scriptsize [0.89, 2.14]} & & {\scriptsize [0.92, 2.69]} & & {\scriptsize [0.6, 1.73]} & & {\scriptsize [1.26, 4.33]} & & {\scriptsize [1.04, 2.79]} & & {\scriptsize [1.12, 3.25]} & \\
% \midrule
% \multirow{2}{*}{Salary Scenario} & \textbf{1.29} & \multirow{2}{*}{\textbf{0.03*}} & \textbf{1.32} & \multirow{2}{*}{\textbf{0.04*}} & 0.80 & \multirow{2}{*}{0.11} & 0.75 & \multirow{2}{*}{0.06} & 1.23 & \multirow{2}{*}{0.1} & 1.14 & \multirow{2}{*}{0.31} \\ 
% & {\scriptsize [1.03, 1.63]} & & {\scriptsize [1.02, 1.71]} & & {\scriptsize [0.61, 1.05]} & & {\scriptsize [0.56, 1.01]} & & {\scriptsize [0.96, 1.57]} & & {\scriptsize [0.88, 1.49]} & \\
% \multirow{2}{*}{Internet Score} & 1.02 & \multirow{2}{*}{0.78} & \textbf{1.17} & \multirow{2}{*}{\textbf{0.04*}} & 1.25 & \multirow{2}{*}{\textbf{0.01**}} & 1.05 & \multirow{2}{*}{0.54} & 1.07 & \multirow{2}{*}{0.36} & 1.01 & \multirow{2}{*}{0.85} \\ 
% & {\scriptsize [0.89, 1.17]} & & {\scriptsize [1.01, 1.36]} & & {\scriptsize [1.06, 1.46]} & & {\scriptsize [0.89, 1.25]} & & {\scriptsize [0.93, 1.23]} & & {\scriptsize [0.87, 1.18]} & \\
 
%  \midrule
%  Moved Org
 Description: & \textbf{1.94} & \multirow{2}{*}{\textbf{0.01*}} & 1.10 & \multirow{2}{*}{0.72} & 1.13 & \multirow{2}{*}{0.59} & 1.71 & \multirow{2}{*}{0.1} & \textbf{1.64} & \multirow{2}{*}{\textbf{0.05*}} & 1.68 & \multirow{2}{*}{0.06} \\ 
~~ \emph{Unsubstantial} & {\scriptsize [1.16, 3.29]} & & {\scriptsize [0.65, 1.86]} & & {\scriptsize [0.73, 1.75]} & & {\scriptsize [0.92, 3.27]} & & {\scriptsize [1.01, 2.67]} & & {\scriptsize [0.99, 2.88]} & \\
Description: & \textbf{1.96} & \multirow{2}{*}{\textbf{0.01*}} & 1.21 & \multirow{2}{*}{0.47} & 1.43 & \multirow{2}{*}{0.1} & \textbf{2.40} & \multirow{2}{*}{\textbf{$<$ 0.01**}} & \textbf{2.15} & \multirow{2}{*}{\textbf{$<$ 0.01**}} & \textbf{2.22} & \multirow{2}{*}{\textbf{$<$ 0.01**}} \\ 
~~ \emph{Techniques} & {\scriptsize [1.17, 3.33]} & & {\scriptsize [0.72, 2.03]} & & {\scriptsize [0.93, 2.22]} & & {\scriptsize [1.33, 4.5]} & & {\scriptsize [1.34, 3.5]} & & {\scriptsize [1.33, 3.77]} & \\
Description: & 1.60 & \multirow{2}{*}{0.08} & 1.05 & \multirow{2}{*}{0.84} & 1.40 & \multirow{2}{*}{0.13} & \textbf{2.06} & \multirow{2}{*}{\textbf{0.02*}} & \textbf{1.76} & \multirow{2}{*}{\textbf{0.02*}} & 1.69 & \multirow{2}{*}{0.05} \\ 
~~ \emph{Enables} & {\scriptsize [0.95, 2.73]} & & {\scriptsize [0.63, 1.77]} & & {\scriptsize [0.91, 2.16]} & & {\scriptsize [1.13, 3.88]} & & {\scriptsize [1.09, 2.87]} & & {\scriptsize [1, 2.9]} & \\
Description: & \textbf{1.86} & \multirow{2}{*}{\textbf{0.02*}} & 1.04 & \multirow{2}{*}{0.89} & 1.43 & \multirow{2}{*}{0.11} & \textbf{1.99} & \multirow{2}{*}{\textbf{0.03*}} & 1.38 & \multirow{2}{*}{0.2} & 1.19 & \multirow{2}{*}{0.55} \\ 
~~ \emph{Trust} & {\scriptsize [1.11, 3.17]} & & {\scriptsize [0.61, 1.76]} & & {\scriptsize [0.92, 2.22]} & & {\scriptsize [1.08, 3.78]} & & {\scriptsize [0.84, 2.28]} & & {\scriptsize [0.68, 2.09]} & \\
Description: & \textbf{2.58} & \multirow{2}{*}{\textbf{$<$ 0.01***}} & \textbf{1.86} & \multirow{2}{*}{\textbf{0.01*}} & 1.43 & \multirow{2}{*}{0.1} & \textbf{2.46} & \multirow{2}{*}{\textbf{$<$ 0.01**}} & \textbf{2.40} & \multirow{2}{*}{\textbf{$<$ 0.01***}} & \textbf{2.27} & \multirow{2}{*}{\textbf{$<$ 0.01**}} \\ 
~~\emph{Risk} & {\scriptsize [1.57, 4.33]} & & {\scriptsize [1.15, 3.05]} & & {\scriptsize [0.93, 2.2]} & & {\scriptsize [1.37, 4.59]} & & {\scriptsize [1.5, 3.88]} & & {\scriptsize [1.37, 3.84]} & \\
Description: & 1.56 & \multirow{2}{*}{0.1} & 1.02 & \multirow{2}{*}{0.95} & 1.38 & \multirow{2}{*}{0.15} & \textbf{2.30} & \multirow{2}{*}{\textbf{0.01**}} & \textbf{1.70} & \multirow{2}{*}{\textbf{0.03*}} & \textbf{1.90} & \multirow{2}{*}{\textbf{0.02*}} \\ 
~~\emph{Technical} & {\scriptsize [0.92, 2.69]} & & {\scriptsize [0.6, 1.73]} & & {\scriptsize [0.89, 2.14]} & & {\scriptsize [1.26, 4.33]} & & {\scriptsize [1.04, 2.79]} & & {\scriptsize [1.12, 3.25]} & \\
\midrule
\multirow{2}{*}{Salary Scenario} & \textbf{1.32} & \multirow{2}{*}{\textbf{0.04*}} & 0.80 & \multirow{2}{*}{0.11} & \textbf{1.29} & \multirow{2}{*}{\textbf{0.03*}} & 0.75 & \multirow{2}{*}{0.06} & 1.23 & \multirow{2}{*}{0.1} & 1.14 & \multirow{2}{*}{0.31} \\ 
& {\scriptsize [1.02, 1.71]} & & {\scriptsize [0.61, 1.05]} & & {\scriptsize [1.03, 1.63]} & & {\scriptsize [0.56, 1.01]} & & {\scriptsize [0.96, 1.57]} & & {\scriptsize [0.88, 1.49]} & \\
\multirow{2}{*}{Internet Score} & \textbf{1.17} & \multirow{2}{*}{\textbf{0.04*}} & \textbf{1.25} & \multirow{2}{*}{\textbf{0.01**}} & 1.02 & \multirow{2}{*}{0.78} & 1.05 & \multirow{2}{*}{0.54} & 1.07 & \multirow{2}{*}{0.36} & 1.01 & \multirow{2}{*}{0.85} \\ 
& {\scriptsize [1.01, 1.36]} & & {\scriptsize [1.06, 1.46]} & & {\scriptsize [0.89, 1.17]} & & {\scriptsize [0.89, 1.25]} & & {\scriptsize [0.93, 1.23]} & & {\scriptsize [0.87, 1.18]} & \\
 
%   \bottomrule
  
% %  P -adjust
%   \toprule
%  \multicolumn{1}{c}{\textbf{Variable}} & \multicolumn{2}{|c}{\textbf{\emph{Hack}}} & \multicolumn{2}{|c}{\textbf{\emph{Law Enforcement}}} & \multicolumn{2}{|c}{\textbf{\emph{\exactexpectationname}}} & \multicolumn{2}{|c}{\textbf{\emph{Data Analyst}}} & \multicolumn{2}{|c}{\textbf{\emph{Graphs}}} & \multicolumn{2}{|c}{\textbf{\emph{Share}}}\\
%  \midrule
%   & OR/CI & p-value & OR/CI & p-value & OR/CI & p-value & OR/CI & p-value & OR/CI & p-value & OR/CI & p-value \\ 
%  \midrule
%  Description: & \textbf{1.94} & \multirow{2}{*}{\textbf{.038}} & 1.10 & \multirow{2}{*}{.788} & 1.13 & \multirow{2}{*}{.662} & 1.71 & \multirow{2}{*}{.150} & \textbf{1.64} & \multirow{2}{*}{\textcolor{red}{\textbf{.091}}} & 1.68 & \multirow{2}{*}{.099} \\ 
% ~~ \emph{Unsubstantial} & {\scriptsize [1.16, 3.29]} & & {\scriptsize [0.65, 1.86]} & & {\scriptsize [0.73, 1.75]} & & {\scriptsize [0.92, 3.27]} & & {\scriptsize [1.01, 2.67]} & & {\scriptsize [0.99, 2.88]} & \\
% Description: & \textbf{1.96} & \multirow{2}{*}{\textbf{.0373}} & 1.21 & \multirow{2}{*}{.562} & 1.43 & \multirow{2}{*}{.150} & \textbf{2.40} & \multirow{2}{*}{\textbf{.0194}} & \textbf{2.15} & \multirow{2}{*}{\textbf{.009}} & \textbf{2.22} & \multirow{2}{*}{\textbf{.0130}} \\ 
% ~~ \emph{Techniques} & {\scriptsize [1.17, 3.33]} & & {\scriptsize [0.72, 2.03]} & & {\scriptsize [0.93, 2.22]} & & {\scriptsize [1.33, 4.5]} & & {\scriptsize [1.34, 3.5]} & & {\scriptsize [1.33, 3.77]} & \\
% Description: & 1.60 & \multirow{2}{*}{.138} & 1.05 & \multirow{2}{*}{.885} & 1.40 & \multirow{2}{*}{.174} & \textbf{2.06} & \multirow{2}{*}{\textcolor{red}{\textbf{.0526}}} & \textbf{1.76} & \multirow{2}{*}{\textcolor{red}{\textbf{.0526}}} & 1.69 & \multirow{2}{*}{.0957} \\ 
% ~~ \emph{Enables} & {\scriptsize [0.95, 2.73]} & & {\scriptsize [0.63, 1.77]} & & {\scriptsize [0.91, 2.16]} & & {\scriptsize [1.13, 3.88]} & & {\scriptsize [1.09, 2.87]} & & {\scriptsize [1, 2.9]} & \\
% Description: & \textbf{1.86} & \multirow{2}{*}{\textcolor{red}{\textbf{.0526}}} & 1.04 & \multirow{2}{*}{.910} & 1.43 & \multirow{2}{*}{.150} & \textbf{1.99} & \multirow{2}{*}{\textcolor{red}{\textbf{.067}}} & 1.38 & \multirow{2}{*}{.258} & 1.19 & \multirow{2}{*}{.627} \\ 
% ~~ \emph{Trust} & {\scriptsize [1.11, 3.17]} & & {\scriptsize [0.61, 1.76]} & & {\scriptsize [0.92, 2.22]} & & {\scriptsize [1.08, 3.78]} & & {\scriptsize [0.84, 2.28]} & & {\scriptsize [0.68, 2.09]} & \\
% Description: & \textbf{2.58} & \multirow{2}{*}{\textbf{.002}} & \textbf{1.86} & \multirow{2}{*}{\textbf{.0388}} & 1.43 & \multirow{2}{*}{.150} & \textbf{2.46} & \multirow{2}{*}{\textbf{.0152}} & \textbf{2.40} & \multirow{2}{*}{\textbf{.002}} & \textbf{2.27} & \multirow{2}{*}{\textbf{.009}} \\ 
% ~~\emph{Risk} & {\scriptsize [1.57, 4.33]} & & {\scriptsize [1.15, 3.05]} & & {\scriptsize [0.93, 2.2]} & & {\scriptsize [1.37, 4.59]} & & {\scriptsize [1.5, 3.88]} & & {\scriptsize [1.37, 3.84]} & \\
% Description: & 1.56 & \multirow{2}{*}{.150} & 1.02 & \multirow{2}{*}{.948} & 1.38 & \multirow{2}{*}{.202} & \textbf{2.30} & \multirow{2}{*}{\textbf{.029}} & \textbf{1.70} & \multirow{2}{*}{\textcolor{red}{\textbf{.073}}} & \textbf{1.90} & \multirow{2}{*}{\textcolor{red}{\textbf{.0514}}} \\ 
% ~~\emph{Technical} & {\scriptsize [0.92, 2.69]} & & {\scriptsize [0.6, 1.73]} & & {\scriptsize [0.89, 2.14]} & & {\scriptsize [1.26, 4.33]} & & {\scriptsize [1.04, 2.79]} & & {\scriptsize [1.12, 3.25]} & \\
% \midrule
% \multirow{2}{*}{Salary Scenario} & \textbf{1.32} & \multirow{2}{*}{\textcolor{red}{\textbf{.076}}} & 0.80 & \multirow{2}{*}{.150} & \textbf{1.29} & \multirow{2}{*}{\textcolor{red}{\textbf{.067}}} & 0.75 & \multirow{2}{*}{.099} & 1.23 & \multirow{2}{*}{.150} & 1.14 & \multirow{2}{*}{.395} \\ 
% & {\scriptsize [1.02, 1.71]} & & {\scriptsize [0.61, 1.05]} & & {\scriptsize [1.03, 1.63]} & & {\scriptsize [0.56, 1.01]} & & {\scriptsize [0.96, 1.57]} & & {\scriptsize [0.88, 1.49]} & \\
% \multirow{2}{*}{Internet Score} & \textbf{1.17} & \multirow{2}{*}{\textcolor{red}{\textbf{.081}}} & \textbf{1.25} & \multirow{2}{*}{\textbf{.025}} & 1.02 & \multirow{2}{*}{.840} & 1.05 & \multirow{2}{*}{.627} & 1.07 & \multirow{2}{*}{.443} & 1.01 & \multirow{2}{*}{.885} \\ 
% & {\scriptsize [1.01, 1.36]} & & {\scriptsize [1.06, 1.46]} & & {\scriptsize [0.89, 1.17]} & & {\scriptsize [0.89, 1.25]} & & {\scriptsize [0.93, 1.23]} & & {\scriptsize [0.87, 1.18]} & \\
 
  \bottomrule
  
  
\end{tabular}
\caption{\small \label{tab:betterbydefn} Logistic regression models of the relationship between the DP description a respondent was shown and their perception of the likelihood that their information will be disclosed through a particular information flow. See Table~\ref{tab:explicityexpectationssharing} for detailed legend.}
\end{table*}

\subsection{RQ2: How Does the Probability of Information Disclosure Influence  Sharing?}\label{sec:explicityexpectationssharing}
Next, we investigate whether setting respondents' expectations about the information disclosures that concerned them influences their reported willingness to share information (Table~\ref{tab:explicityexpectationssharing}).%This would establish that users not only care about information disclosures, but allow such risks to inform their sharing decisions.

Among respondents who care about their information being hacked by a criminal organization or foreign government, those who were told that the risk of this disclosure occurring is about the same as the risk of having their bank account compromised (``Low Risk'' in Table~\ref{tab:explicityexpectationssharing}) are nearly twice (O.R. = $1.91$, $p<0.01$) as likely to share their information as compared to respondents who were told that this risk is greater than the risk of having their bank account compromised. Those who are told there is no risk of their information being disclosed through a hack were nearly three times as likely to share (O.R. = $2.97$, $p<0.01$). Respondents who care about their information being hacked were also more willing to share salary information than medical information.

Respondents that care about information disclosure to the organization running the initiative to which they might contribute their information were $>60\%$ more willing to share if the risk of their information being disclosed to the organization was lower (Low Risk: O.R. = $1.63$, $p=0.01$; No Risk: O.R. = $1.61$, $p=0.01$).

On the other hand, respondents who care about whether law enforcement would be able to access their information with a court order and respondents who care about whether their information might be disclosed to a third-party are both more likely to share their information only if they are told there is no risk of their information being disclosed to these entities. Respondents that are told there is no such risk are about twice as likely to share their information (Law Enforcement: O.R. = $2.07$, $p<0.01$; Share: O.R. = $1.97$, $p<0.01$). Being told there is a low risk instead of a high risk of such a disclosure has no significant effect on their willingness to share. 

We hypothesize that respondents show a graduated response to the risk of information disclosures to the organization running the initiative to which they might contribute their information because it is appropriate for this organization to have their information. Similarly, we hypothesize that respondents show a graduated response to the risk of hacks because information disclosures resulting from hacks are unintentional on the part of the organization. On the other hand, the organization purposefully choosing to share information they contributed to the initiative with a third party or with law enforcement, even with a court order, may feel in-congruent with the purpose for which they shared their information.

Finally, we find that the probability of disclosure to data analysts or through graphs has no effect on willingness to share, even among respondents who care about those information. We hypothesize that those respondents who are motivated by the altruistic goals specified in the scenarios may be willing to share their information regardless of the risk of disclosure occurring through these information flows, which are arguably the most appropriate information flows we examine, while those who are not compelled by the goals of the organizations described in the scenarios are similarly unwilling to share their information regardless of this risk. For example, one respondent who cared about information disclosure to both of these entities, and was told there was no risk of disclosure to a data analyst and low risk of disclosure through a graph said, ``Unfortunately, I do not see enough of a benefit for me to take the risk of sharing my personal information. I absolutely do not want such personal info being leaked out.`` On the other hand, a respondent who cared about disclosure to a data analyst and was told the risk of this disclosure was higher than the risk that their bank account would be compromised commented that they would be willing to share their information, ``because it's for good research, and I'm getting too old to worry about who sees my medical record. I anticipate I will have *many* doctors, nurses, lab techs, etc involved in my medical record before too long.''

We note that respondents who cared about information disclosures to data analysts with higher internet scores were more likely to report being willing to share their information. As technologically savvy respondents, they may have had a clearer mental model of the data analysis process and therefore understood that data analysts typically have complete access to user information. As such, they may be more forgiving toward any approach that aims to reduce this level of access, even given relatively high risk of an information disclosure.% this kind of information leak.

\subsection{RQ3: How Do Differential Privacy Descriptions Affect Privacy Expectations?}\label{sec:expectationsbydefn}

\begin{figure*}[h!t!]
  \centering
  \subfloat[][\scriptsize \label{fig:dist:correct:local}Distribution of respondent correctness about information disclosures under local DP. The x-axis shows percentage of disclosures for which their expectations were correct under local DP.]{\includegraphics[width=.47\textwidth]{distribution_localcorrect.pdf}
  } \hfill
  \subfloat[][\scriptsize \label{fig:dist:correct:central}Distribution of respondent correctness about information disclosures under central DP. The x-axis shows percentage of disclosures for which their expectations were correct under central DP.]{ \includegraphics[width=.47\textwidth]{distribution_centralcorrect.pdf}}
  \caption{\small Influence of in-the-wild descriptions of DP on respondent expectations for information disclosures. Dashed lines are 95\% confidence intervals of the distribution's mean. Respondents could answer ``I don't know'' for all questions; this response is not counted as correct.}
  \label{fig:distributions}
\end{figure*}
% \begin{table*}[!ht]
% \centering%
% \small
% \caption{Scenarios and Expectations used in both Survey One and Survey Two.}

% \label{tab:scenariosandexpectation}
% \begin{tabularx}{\linewidth}{lXcc}
% \toprule
% \textbf{Expectation Name} & \textbf{Expectation Description} & \textbf{Baseline: Local} & \textbf{Baseline: Central} \\
% \midrule
% \midrule

% \multirow{2}{*}{\emph{Exact}} & ``My friend will not be able to learn my salary and job title'' \\\cline{2-2}
% & ``The contents of my medical record will be stored only by my doctor's office, and will not be stored by the non-profit'' & False & False\\
% \midrule

% \smallskip 
% \multirow{2}{*}{\emph{Hack}} & ``A criminal or foreign government that hacks the transparency initiative could learn my salary and job title'' \\\cline{2-2}
% & ``A criminal or foreign government that hacks the non-profit could learn my medical history'' & True & False \\
% \midrule

% \smallskip 
% \multirow{2}{*}{\emph{Law Enforcement}} & ``A law enforcement organization could access my salary and job title with a court order requesting this data from the initiative'' \\\cline{2-2}
% & ``A law enforcement organization could access my medical history with a court order requesting this data from the non-profit'' & True & False \\
% \midrule

% \smallskip 
% \multirow{2}{*}{\emph{Data Analyst}} & ``A data analyst working on the salary transparency initiative could learn my exact salary and job title'' \\\cline{2-2}
% & ``A data analyst working for the non-profit would be able to see my exact medical history'' & True & False \\
% \midrule

% \smallskip 
% \multirow{2}{*}{\emph{Graphs}} & ``Graphs or informational charts created using information given to the salary transparency initiative could reveal my salary and job title.'' \\\cline{2-2}
% & ``Graphs or informational charts created using information given to the non-profit could reveal my medical history.'' & True & True \\
% \midrule

% \smallskip 
% \multirow{2}{*}{\emph{Share}} & ``Data that the salary transparency initiative shares with other organizations doing salary research could reveal my salary and job title'' \\\cline{2-2}
% & ``Data that the non-profit shares with other organizations doing medical research could reveal my medical history'' & True & False \\


% \bottomrule
% \end{tabularx}
% \end{table*}  

We divide our results for RQ3 into two parts. First, we detail our findings regarding the way descriptions of DP \emph{increase} respondents' privacy expectations (see \cref{tab:betterbydefn}). Second, we investigate if the descriptions \emph{correctly} set respondents' privacy expectations, with respect to the ground truth privacy properties of typical local and central DP deployments (see \cref{fig:distributions}).

\medskip \noindent
\textbf{Descriptions Increasing Expectations.} Overall, we find that each description of DP that we tested increased respondents' privacy expectations for at least one of the disclosure risks. However, different descriptions increased different privacy expectations. %compared to the control group (who were not told their data would be protected by DP), respondents who were shown any of the DP descriptions were less likely to think that their data would be leaked through any of the listed flows.

% We find that none of the descriptions of DP influence respondents' perceptions about the whether their data will be leaked to the organization with which they shared the data. Given that neither local nor central DP does effect whether or not the organization with which users share their data can learn their exact data, this is suggests that the descriptions are not over promising on this point.

First, we found that none of the descriptions significantly changed respondents' expectations when it came to disclosing their information to the organization soliciting their information (or their representative). Users did have higher expectations in the salary scenario than in the medical scenario, indicating that the slightly different wording of these expectations may have had an effect on respondent expectations. We verified that this wording did not interfere with our main finding (that no descriptions increased users expectations of the \emph{\exactexpectationname} disclosure) by re-building our models on each dataset; we found the same results.

Four of the descriptions do, however, influence respondents' perceptions regarding whether their information could be disclosed through a hack. Respondents who were shown the \emph{Unsubstantial}, \emph{Techniques}, and \emph{Trust} explanations were nearly two times more likely (\emph{Unsubstantial:} O.R. = 1.94, $p$ = 0.01, \emph{Techniques:} O.R. = 1.96, $p$ = 0.01, \emph{Trust:} O.R. = 1.86, $p$ = 0.02) to think their information would not be disclosed through a hack. Those who were shown the \emph{Risk} description were even more likely (O.R. = 2.58, $p$ < 0.01) to think their information could not be disclosed through a hack. Users may see preventing hacks as one of the key roles of security and privacy technologies, as these results indicate that they expect such protection from the gold standard techniques (\emph{Unsubstantial}) and those used by major companies (\emph{Trust}). The \emph{Risk} description directly addresses this potential information disclosure, so it is unsurprising that it raised privacy expectations regarding hacks. Finally, respondents may have gathered that injecting statistical noise (\emph{Techniques}) would protect their information against hacks, as it does in practice.

Only the \emph{Risk} description significantly influenced respondents' perceptions of whether their information would be disclosed to law enforcement as the result of a court order: those who saw the \emph{Risk} description were nearly two times more likely (O.R. 1.86, $p$ = 0.01) to think their information would not be disclosed to law enforcement. Interestingly, this indicates that users may see information sharing with law enforcement as a risk, rather than an information flow that is appropriate and necessary to protect society. 

All of the descriptions aside from the \emph{Unsubstantial} description increase the likelihood that respondents think their information would be secure against disclosures to a data analyst, while all but the \emph{Trust} description increase the likelihood that respondents think their information would not be disclosed through graphs or charts made using their information. It may be that the \emph{Unsubstantial} description did not raise respondents' expectations for disclosure to data analysts because users are unfamiliar with the notion that a data analysts could accomplish their job without seeing user information --- users may expect even ``gold standard'' techniques to disclose information in this way. Similarly, users may be unfamiliar with the idea that tech companies create graphs and charts, as most of these releases are not customer facing. Therefore, it would not be assumed that such techniques could protect user information.

The \emph{Techniques}, \emph{Risk}, and \emph{Technical} descriptions all increase the likelihood that respondents think their information could not be shared with another organization (\emph{Techniques:} O.R. 2.22, $p$ < 0.01, \emph{Risk:} O.R. 2.27, $p$ < 0.01, \emph{Technical:} O.R. 1.90, $p$ = 0.02). As above, users may have gathered that the injection of statistical noise described in the \emph{Techniques} description would prevent this information disclosure. Additionally, both the \emph{Risks} and \emph{Technical} descriptions speak to the risk of joining the dataset. As indicated in our results for RQ1, a large number of respondents care about their information being disclosed to a third party. This may be a primary ``risk'' in their mind, which the descriptions suggest that they would be secure against.
% Overall, the \emph{Risk} description raised the most expectations. This is intuitive, as the disclosures listed above are all risks of sharing information, and therefore respondents presented with this description may have thought such risks were less likely. \gsk{more?} 
%Interestingly, we also find that respondents were less likely to think salary data would be leaked to the organization or through a hack and we find that those who have higher internet skill are less likely to think their data will be leaked through a hack or to law enforcement. \elissa{I welcome hypotheses, I suspect the internet skill is due to respondents with higher skill having a better sense of the likelihood of these things because they're more common? We could also just drop this}

\smallskip \noindent
\textbf{Descriptions Setting Expectations Correctly.} Not all DP techniques reduce the likelihood of all of these potential information disclosures. It is critical that descriptions of DP are not used only to raise privacy expectations, but, instead, seek to set users' expectations correctly. This is especially important in DP; a potential user encountering a description of a DP may set their expectations as though the system offers local DP, only to discover later that their information was more vulnerable because the deployment used central DP %Thus, we examine both whether these in-the-wild descriptions of DP reduce respondents' expectation that their data will be leaked \textit{and} whether they set respondent expectations correctly 
(see \cref{tab:scenariosandexpectation} for the ground truth we consider under both local and central DP). 


Revisiting our findings above, we note that local DP provides protection against all of the information disclosure risks about which we asked. This is because under local DP the curator never has access to the unperturbed data (and therefore cannot accidentally or intentionally disclose information). As such, increased expectations means more correct expectations under local DP. As we saw above, each of the descriptions does increase some --- but not all --- expectations. This means that the descriptions are not only raising user expectations for differentially private systems, but setting those expectations more accurately.

In central DP, on the other hand, the curator has access to users raw information. In this model, the curator is responsible for injecting statistical noise into any aggregations that are released for public consumption, {\em e.g.} graphs and informational charts. Because the curator has access to raw information, a typical deployment would be able to disclose sensitive information in all of the listed ways, with the exception of \emph{Graphs}. Thus, the descriptions that raise privacy expectations related to \emph{Hack}, \emph{Law Enforcement}, \emph{Data Analyst}, and \emph{Share} disclosures are actually misleading users %with respect to the \emph{Hack}, \emph{Law Enforcement}, \emph{Data Analyst}, and \emph{Share} disclosures 
in the central model.


Finally, we also consider the aggregate effect of the descriptions we study on the accuracy of respondents' privacy expectations (see \cref{fig:distributions}). We find that respondents' expectations of DP are more in line with the central model than the local model (that is, they have lower privacy expectations). Specifically, respondents had correctly set expectations for less than half of the information disclosure risks under local DP, while roughly half of their expectations were set correctly for the central model. More importantly, we note that users' privacy expectations are poorly aligned with \emph{both} local and central DP. This indicates that users do not have a coherent mental model of the data collection process, as many of the privacy expectations about which we ask are equivalent from a technical perspective.
%
% Local DP can prevent users exact data from being leaked during a hack, while central DP cannot. Thus, some of the descriptions are appropriately setting respondent expectations under local DP while others are correctly setting expectations under central DP, although none of the descriptions specify the setting \elissa{or something? Gabe/Rachel maybe check which descriptions are supposed to be about what and say more?}
%
% Given that local DP can protect against law enforcement learning respondents' exact data while central DP cannot, this means that only the risk description is setting respondent expectations correctly for local DP. \elissa{feel free to add hypotheses about why if appropriate, alternately in discussion we can use all this as support about the fact that these descriptions are setting expectations all over the map / not effectively. so basically, they do influence things, but not usefully; then we can use the other usenix paper as support that if you do it well, it can be effective. and an alternative to training people on it is to set expectations via data flows}
%
% Local DP can prevent both leaks to the data analyst and through graphs, while central DP can only prevent leaks through graphs. Thus, the unsubstantial description does set respondent expectations correctly under central DP, but the trust description does not set respondent expectations correctly under either local or central DP. \elissa{I think? check that my correctness stuff is correct please, ha!}
% GABE HERE FLIPPED TABLE
% \begin{table*}[ht]
% \centering
% \small
% \label{tab:worsebydefn}
% \begin{tabular}{lrl|rl|rl|rl|rl|rl} 
%  \toprule
%  \multicolumn{1}{c}{\textbf{Variable}} & \multicolumn{2}{|c}{\textbf{\emph{Exact}}} & \multicolumn{2}{|c}{\textbf{\emph{Hack}}} & \multicolumn{2}{|c}{\textbf{\emph{Law Enforcement}}} & \multicolumn{2}{|c}{\textbf{\emph{Data Analyst}}} & \multicolumn{2}{|c}{\textbf{\emph{Graphs}}} & \multicolumn{2}{|c}{\textbf{\emph{Share}}}\\
%  \midrule
%  & OR & p-value & OR & p-value & OR & p-value & OR & p-value & OR & p-value & OR & p-value \\ 
%  \midrule
%  Description: \emph{Unsubstantial}& 0.79 & 0.3 & 0.70 & 0.11 & 0.79 & 0.3 & 0.66 & 0.08 & 0.63 & 0.04* & 0.72 & 0.16 \\ 
%  Description: \emph{Techniques}	 & 0.90 & 0.64 & 0.60 & 0.02* & 0.63 & 0.03* & 0.60 & 0.03* & 0.51 & $<$ 0.01** & 0.40 & $<$ 0.01*** \\ 
% Description: \emph{Enables} 		& 0.79 & 0.29 & 0.85 & 0.47 & 0.86 & 0.5 & 0.64 & 0.06 & 0.60 & 0.02* & 0.61 & 0.03* \\ 
%  Description: \emph{Trust} 			& 0.84 & 0.43 & 0.76 & 0.22 & 0.89 & 0.62 & 0.87 & 0.55 & 0.77 & 0.24 & 0.81 & 0.38 \\ 
% Description: \emph{Risk} 			& 0.88 & 0.56 & 0.41 & $<$ 0.01*** & 0.47 & $<$ 0.01*** & 0.47 & $<$ 0.01** & 0.46 & $<$ 0.01*** & 0.47 & $<$ 0.01*** \\ 
% Description: \emph{Technical} 		& 0.92 & 0.72 & 0.63 & 0.04* & 0.85 & 0.46 & 0.47 & $<$ 0.01** & 0.58 & 0.01* & 0.55 & 0.01** \\ 
% \midrule
% Salary Scenario & 1.15 & 0.25 & 0.93 & 0.57 & 1.44 & $<$ 0.01** & 1.27 & 0.05* & 0.92 & 0.49 & 0.85 & 0.19 \\ 
% Internet Score & 0.94 & 0.39 & 0.81 & $<$ 0.01** & 0.83 & 0.01** & 1.03 & 0.63 & 0.94 & 0.34 & 0.98 & 0.81 \\ 
 %
%  \bottomrule
% \end{tabular}
% \caption{FLIPPED TABLE 4. See Table~\ref{tab:careshare} for detailed legend. }
% \end{table*}
% \subsection{Survey One Results}
% Our first survey attempts to investigate how different descriptions of DP impact user, both in terms of willingness to share data and concrete privacy expectations from a differentially private systems.
%
% \medskip \noindent
% \textbf{DP is not enough to increase willingness to sharing.} We found that respondents were not significantly more willing to share their data when told that the organization holding their data would be using DP (see \cref{tab:sharewithdp}). We note that this result contradicts prior work in this area \cite{SP:XWLJ20}. We believe that this shows how little is known about differentially private messaging. Moreover, it demonstrates that the exact way in which DP is described and the context in which it is described makes a big difference.

\subsection{RQ4: How Do In-The-Wild Descriptions of Differential Privacy Affect Sharing?}\label{sec:sharingbydescriptions}

When analyzing the results of our second survey, we find that respondents who were told that their information would be protected by DP techniques, as described by one of six different descriptions of those techniques, were no more likely to report that they would share their information in either scenario (Table~\ref{tab:sharewithdp}). We also note that the descriptions did not decrease the likelihood that respondents would be willing to share their information. Respondents were, however, more likely (O.R. = 1.67, $p$ < 0.01) to share their information in the salary scenario than in the medical scenario, in line with prior work suggesting that medical information is particularly sensitive~\cite{ion2011home}. 

We note that this finding contradicts the findings of \cite{SP:XWLJ20}, who found that DP increased respondents' willingness to share high sensitivity information. We note that (A) the ways in which we describe DP and (B) the context in which we elicit responses are different. As discussed in \cref{sec:sppaperbackground}, the descriptions used in this prior work were significantly longer and not necessarily representative of in-the-wild descriptions from which we derived our descriptions, and the methodology of prior work also involved mechanisms to ensure respondents correctly understood the privacy guarantees detailed in the descriptions.% We believe that this indicates that their results may not generalize well in practice, where users are likely to be given brief descriptions of DP like the ones we use.


\begin{table}[t!]
\centering

\small
\begin{tabular}{lrll}
 \toprule
%\multicolumn{4}{c}{\textbf{Sharing Information With Different Descriptions}} \\
 %\midrule
 Variable & Odds Ratio & CI & p-value \\ 
 \midrule
 Description: \emph{Unsubstantial}	& 1.22 & [0.79, 1.88] & 0.37 \\
 Description: \emph{Techniques} 	& 0.96 & [0.62, 1.47] & 0.83 \\
 Description: \emph{Enables} 	 & 1.48 & [0.96, 2.29] & 0.08 \\
 Description: \emph{Trust} 		 	& 1.08 & [0.7, 1.67] & 0.72 \\
 Description: \emph{Risk} 			& 1.37 & [0.89, 2.12] & 0.15 \\
 Description: \emph{Technical} 		& 0.94 & [0.61, 1.45] & 0.77 \\
 \midrule
Salary Scenario & \textbf{1.67} & \textbf{[1.32, 2.1]} & $<$ \textbf{0.01***} \\ 
Internet Score & 1.09 & [0.95, 1.25] & 0.2 \\
  \bottomrule
\end{tabular}
\caption{\small \label{tab:sharewithdp} Logistic regression showing the effect of the descriptions of DP on respondents' likelihood of being willing to share information.}
\end{table}

==> tablesatend.tex <==
\clearpage
\section{Tables}


\begin{table*}[ht]
\centering
\caption{Sharing with better expectations}
\small
\label{tab:sharingbyexpectationsanddefinitions}
\begin{tabular}{lrll}
  \toprule
\multicolumn{4}{c}{\textbf{Sharing Data With Higher Expectations}} \\
  \midrule
  Variable & Odds Ratio & CI & p value \\ 
  \midrule
Higher \emph{Exact} Expectation  						& \textbf{2.38} & \textbf{[1.84, 3.1]} & $<$ \textbf{0.01***} \\ 
Higher \emph{Hack} Expectation 	 			& \textbf{2.07} & \textbf{[1.5, 2.87]} & $<$ \textbf{0.01***} \\ 
Higher \emph{Law Enforcement} Expectation		 & \textbf{1.55} & \textbf{[1.11, 2.17]} & \textbf{0.01*} \\ 
Higher \emph{Data Analyst} Expectation 	 		& \textbf{0.52} & \textbf{[0.36, 0.74]} & $<$ \textbf{0.01***} \\ 
Higher \emph{Graphs} Expectation  				& \textbf{1.47} & \textbf{[1.09, 1.98]} & \textbf{0.01*} \\ 
Higher \emph{Share} Expectation  						& \textbf{2.55} & \textbf{[1.82, 3.62]} & $<$ \textbf{0.01***} \\ 
 \midrule
Salary Scenario & \textbf{1.55} & \textbf{[1.21, 1.99]} & $<$ \textbf{0.01***} \\ 
Internet Score & 1.06 & [0.92, 1.22] & 0.42 \\ 
   \bottomrule
\end{tabular}
\end{table*}




\begin{table*}[ht]
\centering
\caption{This is a caption}
\small
\label{tab:sharingbyexpectationsanddefinitions}
\begin{tabular}{lrll|lrll}
  \toprule
  \multicolumn{4}{c|}{\textbf{Sharing Data With Higher Expectations}} & \multicolumn{4}{c}{\textbf{Sharing Data With Different Descriptions}} \\
  \midrule
  Variable & Odds Ratio & CI & p value & Variable & Odds Ratio & CI & p value \\ 
  \midrule
%  (Intercept) & 0.24 & [0.13, 0.45] & $<$ 0.01*** &  (Intercept) & 0.41 & [0.22, 0.76] & 0.01** \\ 
 Higher \emph{Exact} Expectation & \textbf{2.39} & \textbf{[1.83, 3.15]} & $<$ \textbf{0.01***} &  Description: \emph{Unsubstantial} & 1.29 & [0.83, 2.03] & 0.26 \\
 Higher \emph{Hack} Expectation & \textbf{1.88} & \textbf{[1.35, 2.62]} & $<$ \textbf{0.01***} &  Description: \emph{Techniques} & 1.07 & [0.68, 1.67] & 0.78 \\
 Higher \emph{Law Enforcement} Expectation & \textbf{1.55} & \textbf{[1.1, 2.2]} & \textbf{0.01*} & Description: \emph{Enables} & \textbf{1.76} & \textbf{[1.11, 2.8]} & \textbf{0.02*} \\
 Higher \emph{Data Analyst} Expectation & \textbf{0.52} & \textbf{[0.36, 0.76]} & $<$ \textbf{0.01***} &  Description: \emph{Trust} & 1.14 & [0.73, 1.79] & 0.56 \\
 Higher \emph{Graphs} Expectation & \textbf{1.46} & \textbf{[1.08, 1.99]} & \textbf{0.02*} & Description: \emph{Risk} & 1.44 & [0.92, 2.26] & 0.11 \\
 Higher \emph{Share} Expectation & \textbf{2.56} & \textbf{[1.8, 3.68]} & \textbf{$<$ 0.01***} & Description: \emph{Technical} & 1.05 & [0.67, 1.65] & 0.83 \\
 \midrule
 Salary Scenario & \textbf{1.56} & \textbf{[1.2, 2.02]} & $<$ \textbf{0.01***} &  Salary Scenario & \textbf{1.65} & \textbf{[1.29, 2.1]} & $<$ \textbf{0.01***} \\ 
 Internet Score & 1.06 & [0.91, 1.23] & 0.43 &  Internet Score & 1.09 & [0.94, 1.25] & 0.25 \\ 
 Gender: woman & 0.81 & [0.62, 1.05] & 0.12 &  Gender: woman & 0.74 & [0.58, 0.95] & 0.02* \\ 
 Race: black & 0.97 & [0.65, 1.44] & 0.86 &  Race: black & 0.90 & [0.62, 1.31] & 0.58 \\ 
 Race: asian & \textbf{0.43} & \textbf{[0.26, 0.71]} & $<$ \textbf{0.01**} &  Race: asian & \textbf{0.36} & \textbf{[0.22, 0.58]} & $<$ \textbf{0.01***} \\ 
 Race: hispanic & 0.66 & [0.4, 1.09] & 0.11 &  Race: hispanic & 0.68 & [0.42, 1.08] & 0.1 \\ 
 Race: native american & 0.83 & [0.26, 2.81] & 0.76 &  Race: native american & 1.25 & [0.42, 3.98] & 0.69 \\ 
 Edu: Some College & 1.13 & [0.69, 1.87] & 0.63 &  Edu: Some College & 1.24 & [0.78, 1.97] & 0.38 \\ 
 Edu: Bachelors+ & 1.56 & [0.98, 2.48] & 0.06 &  Edu: Bachelors+ & \textbf{1.92} & \textbf{[1.24, 2.98]} & $<$ \textbf{0.01**} \\ 
  Income: \$30k-\$50k & \textbf{1.75} & \textbf{[1.17, 2.61]} & \textbf{0.01**} &  Income: \$30k-\$50k & \textbf{1.62} & \textbf{[1.12, 2.35]} & \textbf{0.01*} \\ 
 Income: \$50k-\$100k & \textbf{1.69} & \textbf{[1.16, 2.46]} & \textbf{0.01**} &  Income: \$50k-\$100k & \textbf{1.49} & \textbf{[1.05, 2.11]} & \textbf{0.03*} \\ 
 Income: \$100k-\$200k & \textbf{1.84} & \textbf{[1.11, 3.04]} & \textbf{0.02*} &  Income: \$100k-\$200k & 1.42 & [0.89, 2.27] & 0.14 \\ 
 Income: \$200k+ & 2.49 & [0.98, 6.74] & 0.06 &  Income: \$200k+ & 2.05 & [0.85, 5.34] & 0.12 \\ 
   \bottomrule
\end{tabular}
\end{table*}

\begin{table*}[ht]
\centering
\caption{SALARY DATA ONLY This is a caption}
\small
\label{tab:sharingbyexpectationsanddefinitions}
\begin{tabular}{lrll|lrll}
  \toprule
  \multicolumn{4}{c|}{\textbf{Sharing Data With Higher Expectations}} & \multicolumn{4}{c}{\textbf{Sharing Data With Different Descriptions}} \\
  \midrule
  Variable & Odds Ratio & CI & p value & Variable & Odds Ratio & CI & p value \\ 
  \midrule
Higher \emph{Exact} Expectation               & \textbf{2.63} & \textbf{[1.77, 3.93]} & $<$ \textbf{0.01***} &       Description: \emph{Unsubstantial}   & 0.79 & [0.42, 1.5] & 0.47 \\ 
Higher \emph{Hack} Expectation              & \textbf{1.76} & \textbf{[1.11, 2.84]} & \textbf{0.02*} &              Description: \emph{Techniques}       & 0.91 & [0.47, 1.73] & 0.76 \\ 
Higher \emph{Law Enforcement} Expectation  & 1.32 & [0.79, 2.24] & 0.3 &                  Description: \emph{Enables}           & \textbf{2.28} & \textbf{[1.11, 4.81]} & \textbf{0.03*} \\ 
Higher \emph{Data Analyst} Expectation  & \textbf{0.44} & \textbf{[0.25, 0.78]} & $<$ \textbf{0.01**} &              Description: \emph{Trust}            & 1.18 & [0.61, 2.27] & 0.62 \\ 
Higher \emph{Graphs} Expectation            & \textbf{1.59} & \textbf{[1.03, 2.47]} & \textbf{0.04*} &               Description: \emph{Risk}          & 1.46 & [0.75, 2.86] & 0.26 \\ 
Higher \emph{Share} Expectation            & \textbf{1.63} & \textbf{[1.01, 2.69]} & \textbf{0.05*} &                Description: \emph{Technical}         & 1.26 & [0.65, 2.43] & 0.49 \\ 
\midrule
Internet Score  & 1.23 & [0.99, 1.54] & 0.07 &              Internet Score             & 1.24 & [1, 1.54] & 0.06 \\ 
Gender: woman                & 0.81 & [0.55, 1.18] & 0.27 &                  Gender: woman              & 0.78 & [0.54, 1.12] & 0.18 \\ 
Race: black                  & 1.28 & [0.71, 2.36] & 0.43 &                  Race: black                  & 1.17 & [0.67, 2.12] & 0.59 \\ 
Race: asian                  & 0.64 & [0.3, 1.38] & 0.25 &                   Race: asian              & 0.56 & [0.27, 1.18] & 0.12 \\ 
Race: hispanic               & 0.66 & [0.35, 1.28] & 0.22 &               Race: hispanic             & 0.58 & [0.31, 1.1] & 0.09 \\ 
Race: native american        & 1.02 & [0.23, 5.7] & 0.98 &            Race: native american        & 1.19 & [0.31, 5.91] & 0.81 \\ 
Edu: Some College            & 1.20 & [0.59, 2.42] & 0.62 &                Edu: Some College          & 1.52 & [0.78, 2.98] & 0.22 \\ 
Edu: Bachelors+               & 1.87 & [1, 3.53] & 0.05 &                  Edu: Bachelors+            & \textbf{2.14} & \textbf{[1.17, 3.93]} & \textbf{0.01*} \\ 
Income: \$30k-\$50k           & 1.66 & [0.93, 2.98] & 0.09 &         Income: \$30k-\$50k        & 1.53 & [0.88, 2.66] & 0.13 \\ 
Income: \$50k-\$100k         & 1.49 & [0.87, 2.56] & 0.15 &        Income: \$50k-\$100k        & 1.35 & [0.8, 2.26] & 0.26 \\ 
Income: \$100k-\$200k       & 1.77 & [0.84, 3.83] & 0.14 &       Income: \$100k-\$200k     & 1.70 & [0.83, 3.59] & 0.15 \\ 
Income: \$200k+              & 1.78 & [0.39, 9.75] & 0.47 &          Income: \$200k+            & 1.43 & [0.34, 7.42] & 0.64 \\ 
   \bottomrule
\end{tabular}
\end{table*}


\begin{table*}[ht]
\centering
\caption{MEDICAL DATA ONLY This is a caption}
\small
\label{tab:sharingbyexpectationsanddefinitions}
\begin{tabular}{lrll|lrll}
  \toprule
  \multicolumn{4}{c|}{\textbf{Sharing Data With Higher Expectations}} & \multicolumn{4}{c}{\textbf{Sharing Data With Different Descriptions}} \\
  \midrule
  Variable & Odds Ratio & CI & p value & Variable & Odds Ratio & CI & p value \\ 
  \midrule
Higher \emph{Exact} Expectation               &  \textbf{2.45} & \textbf{[1.65, 3.65]} & $<$ \textbf{0.01***}        & Description: \emph{Unsubstantial}  & \textbf{2.30} & \textbf{[1.21, 4.43]} & \textbf{0.01*} \\ 
Higher \emph{Hack} Expectation              & \textbf{1.99} & \textbf{[1.24, 3.23]} & \textbf{0.01**}               & Description: \emph{Techniques}      & 1.36 & [0.72, 2.57] & 0.34 \\ 
Higher \emph{Law Enforcement} Expectation & 1.70 & [1.06, 2.75] & 0.03*                  &  Description: \emph{Enables}        & 1.57 & [0.84, 2.95] & 0.16 \\ 
Higher \emph{Data Analyst} Expectation    & 0.55 & [0.33, 0.92] & 0.02*                  &    Description: \emph{Trust}         & 1.21 & [0.63, 2.32] & 0.56 \\ 
Higher \emph{Graphs} Expectation          & 1.36 & [0.87, 2.13] & 0.18                   &  Description: \emph{Risk}            & 1.48 & [0.79, 2.8] & 0.22 \\ 
Higher \emph{Share} Expectation             & \textbf{4.09} & \textbf{[2.44, 7.04]} & $<$ \textbf{0.01***}          &  Description: \emph{Technical}     & 0.87 & [0.45, 1.66] & 0.67 \\ 
\midrule
Internet Score                              & 0.94 & [0.76, 1.16] & 0.56                 & Internet Score         & 0.96  & [0.79, 1.17] & 0.68 \\ 
Gender: woman                             & 0.86 & [0.58, 1.25] & 0.42                   & Gender: woman          & 0.73 & [0.51, 1.04] & 0.08 \\ 
Race: black                               & 0.75 & [0.42, 1.33] & 0.33                   & Race: black            & 0.70 & [0.41, 1.17] & 0.18 \\ 
Race: asian                               & \textbf{0.33} & \textbf{[0.15, 0.67]} & $<$ \textbf{0.01**}             & Race: asian              & \textbf{0.24} & \textbf{[0.12, 0.46]} & $<$ \textbf{0.01***} \\ 
Race: hispanic                            & 0.64 & [0.29, 1.43] & 0.28                   & Race: hispanic         & 0.83 & [0.4, 1.72] & 0.62 \\ 
Race: native american                    & 0.62 & [0.07, 4.64] & 0.65                    & Race: native american   & 1.52 & [0.17, 10.27] & 0.68 \\ 
Edu: Some College                          & 1.00 & [0.47, 2.12] & 0.99                  & Edu: Some College       & 0.97 & [0.49, 1.91] & 0.92 \\ 
Edu: Bachelors+                            & 1.25 & [0.61, 2.57] & 0.54                  & Edu: Bachelors+        & 1.60 & [0.83, 3.08] & 0.16 \\ 
Income: \$30k-\$50k                      & 1.66 & [0.94, 2.94] & 0.08                    & Income: \$30k-\$50k    & 1.65 & [0.98, 2.78] & 0.06 \\ 
Income: \$50k-\$100k                       & \textbf{1.77} & \textbf{[1.03, 3.04]} & \textbf{0.04*}                 & Income: \$50k-\$100k      & 1.60 & [0.98, 2.62] & 0.06 \\ 
Income: \$100k-\$200k                      & 1.86 & [0.93, 3.75] & 0.08                  & Income: \$100k-\$200k    & 1.18 & [0.62, 2.26] & 0.62 \\ 
Income: \$200k+                            & 2.68 & [0.82, 9.8] & 0.11                   & Income: \$200k+          & 2.45 & [0.8, 8.48] & 0.13 \\  
   \bottomrule
\end{tabular}
\end{table*}

\clearpage



\begin{table*}[ht]
\centering
\caption{Better by Definition}
\small
\label{tab:betterbydefn}
\begin{tabular}{lrl|rl|rl|rl|rl|rl} 
  \toprule
  \multicolumn{1}{c}{\textbf{Variable}}  & \multicolumn{2}{|c}{\textbf{\emph{Exact}}} & \multicolumn{2}{|c}{\textbf{\emph{Hack}}} & \multicolumn{2}{|c}{\textbf{\emph{Law Enforcement}}} & \multicolumn{2}{|c}{\textbf{\emph{Data Analyst}}} & \multicolumn{2}{|c}{\textbf{\emph{Graphs}}} & \multicolumn{2}{|c}{\textbf{\emph{Share}}}\\
  \midrule
   & OR & p value & OR  & p value  & OR  & p value & OR  & p value & OR  & p value & OR  & p value  \\ 
  \midrule
% (Intercept) & 0.29 & $<$ 0.01***  			& 0.09 & $<$ 0.01***  		&  0.15 & $<$ 0.01***    &  0.09 & $<$ 0.01***  		& 0.25 & $<$ 0.01***  		&  0.20 & $<$ 0.01 \\
  Description: \emph{Unsubstantial} & 1.15  & 0.55  		& \textbf{1.95}  & \textbf{0.01*}  			&  1.14 & 0.62     		 &  1.62 & 0.14  				& \textbf{1.67} & \textbf{0.04*}  			&  1.65 & 0.07   \\
  Description: \emph{Techniques} & 1.56  & 0.05  		& \textbf{1.99}  & \textbf{0.01*}  			&  1.20 & 0.5      		 &  \textbf{2.36} & \textbf{0.01**}  				& \textbf{2.27} & $<$ \textbf{0.01***}  		&  \textbf{2.30} & $<$ \textbf{0.01**} \\
 Description: \emph{Enables} & 1.47  & 0.09  		& 1.69 & 0.06  				&  1.07 & 0.79     		 &  \textbf{1.91} & \textbf{0.04*}  				& \textbf{1.66} & \textbf{0.05*}  			&  1.59 & 0.09   \\
  Description: \emph{Trust} & 1.48 & 0.09  			& \textbf{1.92}  & \textbf{0.02*}  			&  1.06 & 0.84     		 &  \textbf{2.02} & \textbf{0.03*}  				& 1.38 & 0.21  				&  1.20 & 0.52   \\
 Description: \emph{Risk} & 1.41  & 0.13  			& \textbf{2.61}  & $<$ \textbf{0.01***} 		&  \textbf{1.84} & \textbf{0.02*}    		 &  \textbf{2.34} & \textbf{0.01**}  				& \textbf{2.37} & \textbf{$<$ 0.01***}  		&  \textbf{2.27} & $<$ \textbf{0.01**} \\
 Description: \emph{Technical} & 1.46  & 0.1  		& 1.64  & 0.08  			&  0.99 & 0.97     		 &  \textbf{2.24} & \textbf{0.01*}  				& \textbf{1.68} & \textbf{0.04*}  			&  \textbf{1.86} & \textbf{0.02*}   \\
 \midrule
  Salary Scenario & 1.22 &  0.09  			& 1.27  & 0.08  			&  0.79 & 0.1      		 &  0.77 & 0.09  				& 1.22 & 0.12  				&  1.11 & 0.46   \\
 Internet Score & 1.00 &   0.99  			& 1.17  & 0.06  			&  \textbf{1.24} & \textbf{0.01*}    		 &  1.07 & 0.43  				& 1.08 & 0.32  				&  1.03 & 0.69   \\
 Gender: woman & 0.94  & 0.61  					& \textbf{0.69} & \textbf{0.01**}  			&  0.81 & 0.14     		 &  0.86 & 0.34  				& \textbf{0.66} & $<$ \textbf{0.01**}  		&  \textbf{0.69} & \textbf{0.01**}   \\
 Race: black & 1.12  & 0.53  					& 0.90  & 0.63  			&  0.78 & 0.28     		 &  0.81 & 0.41  				& \textbf{0.56} & \textbf{0.01**}  			&  0.78 & 0.27   \\
 Race: asian & 0.96 & 0.86  					& \textbf{0.33}  & $<$ \textbf{0.01**}  		&  \textbf{0.50} & \textbf{0.03*}    		 &  0.96 & 0.89  				& 0.86 & 0.56  				&  0.63 & 0.12   \\
 Race: hispanic & 0.68 &  0.11  				& 0.97  & 0.92  			&  1.28 & 0.35     		 &  1.54 & 0.11  				& 1.09 & 0.73  				&  1.47 & 0.13   \\
 Race: native american & \textbf{3.35} &  \textbf{0.03*}  			& 1.07  & 0.92  			&  2.18 & 0.16     		 &  0.66 & 0.59  				& 1.37 & 0.57  				&  1.92 & 0.23   \\
  Edu: Some College & 1.10 &  0.7  				& 1.52  & 0.15  			&  1.69 & 0.08     		 &  1.53 & 0.16  				& 1.30 & 0.31  				&  1.19 & 0.53   \\
 Edu: Bachelor+ & \textbf{1.77} &  \textbf{0.01*}  				& \textbf{1.74}  & \textbf{0.04*}  			&  1.54 & 0.12     		 &  0.93 & 0.8  				& 1.18 & 0.48  				&  1.21 & 0.46   \\
 Income: \$30k-\$50K & \textbf{1.59} & \textbf{0.01*}  		& 1.11 & 0.61  				&  0.89 & 0.58     		 &  1.32 & 0.25  				& 0.90 & 0.59  				&  0.68 & 0.08   \\
 Income: \$50k-\$100K & 1.08 & 0.66  		& 1.07 & 0.73  				&  0.87 & 0.51     		 &  1.29 & 0.27  				& 0.85 & 0.37  				&  0.89 & 0.55   \\
 Income: \$100k-\$200k & 0.72 &  0.18  		& 0.93  & 0.79  			&  0.72 & 0.25     		 &  1.16 & 0.62  				& 0.79 & 0.35  				&  0.87 & 0.61   \\
 Income: \$200k+ & 1.50 &  0.35  			& 0.83  & 0.72  			&  0.82 & 0.69     		 &  \textbf{3.24} & \textbf{0.01*}  				& 1.65 & 0.25  				&  0.95 & 0.91   \\

  
   \bottomrule
\end{tabular}
\end{table*}



\begin{table*}[ht]
\centering
\caption{SALARY ONLY VERSION Better by Definition}
\small
\label{tab:betterbydefn}
\begin{tabular}{lrl|rl|rl|rl|rl|rl} 
  \toprule
  \multicolumn{1}{c}{\textbf{Variable}}  & \multicolumn{2}{|c}{\textbf{\emph{Exact}}} & \multicolumn{2}{|c}{\textbf{\emph{Hack}}} & \multicolumn{2}{|c}{\textbf{\emph{Law Enforcement}}} & \multicolumn{2}{|c}{\textbf{\emph{Data Analyst}}} & \multicolumn{2}{|c}{\textbf{\emph{Graphs}}} & \multicolumn{2}{|c}{\textbf{\emph{Share}}}\\
  \midrule
   & OR & p value & OR  & p value  & OR  & p value & OR  & p value & OR  & p value & OR  & p value  \\ 
  \midrule
Description: \emph{Unsubstantial} 	&1.36 &0.34 & 1.99 & 0.08 & 1.15 &0.74 & 2.57 &0.09 & 1.73 & 0.13 & 1.34 &0.47 \\ 
Description: \emph{Techniques} &1.55 &0.18 & \textbf{2.17} & \textbf{0.05*} & 1.26 &0.57 & \textbf{4.76} &$<$ \textbf{0.01**} & \textbf{2.90} & $<$ \textbf{0.01**} & \textbf{2.48} & \textbf{0.02*} \\ 
Description: \emph{Enables} & 1.56 &0.18 & \textbf{2.22} & \textbf{0.04*} & 1.20 &0.65 & 2.13 &0.19 & 1.68 & 0.16 & 1.65 &0.21 \\ 
Description: \emph{Trust}  & 1.55 &0.18 & \textbf{3.09} & $<$ \textbf{0.01**} & 1.26 &0.56 & \textbf{3.19} & \textbf{0.03*} & 1.88 & 0.08& 1.49 &0.31 \\ 
Description: \emph{Risk} &1.63 &0.13 & \textbf{3.30} & $<$ \textbf{0.01**} & \textbf{2.35} & \textbf{0.03*} & \textbf{4.61} &$<$ \textbf{0.01**} & \textbf{2.60} & \textbf{0.01**} & \textbf{2.66} & \textbf{0.01**} \\ 
Description: \emph{Technical} & 1.62 &0.14 & 2.13 & 0.05 & 1.09 &0.83 & \textbf{3.21} & \textbf{0.03*} & 1.87 & 0.08& 1.99 &0.07 \\ 
\midrule
Internet Score 	&1.09 &0.43 & \textbf{1.26} & \textbf{0.04*} & \textbf{1.53} & $<$ \textbf{0.01**} & \textbf{1.37} & \textbf{0.03*} & 1.19 & 0.11& 1.06 &0.62 \\ 
Gender: woman 		&1.15 &0.42 & 0.75 & 0.13 & 0.72 &0.14 & 1.05 &0.82 & \textbf{0.69} & \textbf{0.05*} & 0.69 &0.06 \\ 
Race: black 	&1.30 &0.33 & 1.08 & 0.79 & 0.66 &0.27 & 1.12 &0.77 & \textbf{0.48} & \textbf{0.03*} & 0.71 &0.31 \\ 
Race: asian 	&1.17 &0.66 & 0.57 & 0.21 & 0.69 &0.43 & 2.21 &0.06 & 1.57 & 0.22& 0.97 &0.94 \\ 
Race: hispanic 		& 0.61 &0.13 & 0.86 & 0.68 & 0.72 &0.42 & \textbf{2.12} & \textbf{0.04*} & 1.42 & 0.28& 1.32 &0.43 \\ 
Race: native american  & 3.13 &0.12 & 1.11 & 0.89 & 1.68 &0.46 & 0.48 &0.51 & 1.03 & 0.96& 0.94 &0.93 \\ 
Edu: Some College 		 &\textbf{2.25} & \textbf{0.02*} & 1.88 & 0.13 & \textbf{2.55} & \textbf{0.03*} & 1.41 &0.46 & 0.97 & 0.94& 1.38 &0.42 \\ 
Edu: Bachelor+ 		 & \textbf{2.10} & \textbf{0.02*} & 1.62 & 0.21 & 1.43 &0.38 & 1.07 &0.88 & 0.90 & 0.73& 1.43 &0.33 \\ 
Income: \$30k-\$50K 	 & 1.50 &0.13 & 1.27 & 0.44 & \textbf{0.45} & \textbf{0.01*} & 0.78 &0.49 & \textbf{0.54} & \textbf{0.03*} & \textbf{0.48} & \textbf{0.01*} \\ 
Income: \$50k-\$100K &1.07 &0.8 & 1.45 & 0.21 & \textbf{0.55} & \textbf{0.04*} & 0.80 &0.51 & 0.67 & 0.13& \textbf{0.55} & \textbf{0.03*} \\ 
Income: \$100k-\$200k 	& 1.11 &0.77 & 1.62 & 0.21 & 0.50 &0.1 & 0.80 &0.63 & 0.76 & 0.45& 0.83 &0.62 \\ 
Income: \$200k+ 	 &2.26 &0.24 & 0.38 & 0.37 & 0.60 &0.55 & 1.36 &0.73 & 1.01 & 0.99& 0.48 &0.38 \\ 
  
   \bottomrule
\end{tabular}
\end{table*}




\begin{table*}[ht]
\centering
\caption{MEDICAL ONLY VERSION Better by Definition}
\small
\label{tab:betterbydefn}
\begin{tabular}{lrl|rl|rl|rl|rl|rl} 
  \toprule
  \multicolumn{1}{c}{\textbf{Variable}}  & \multicolumn{2}{|c}{\textbf{\emph{Exact}}} & \multicolumn{2}{|c}{\textbf{\emph{Hack}}} & \multicolumn{2}{|c}{\textbf{\emph{Law Enforcement}}} & \multicolumn{2}{|c}{\textbf{\emph{Data Analyst}}} & \multicolumn{2}{|c}{\textbf{\emph{Graphs}}} & \multicolumn{2}{|c}{\textbf{\emph{Share}}}\\
  \midrule
   & OR & p value & OR  & p value  & OR  & p value & OR  & p value & OR  & p value & OR  & p value  \\ 
  \midrule
Description: \emph{Unsubstantial} & 1.43& 0.28  & 1.35& 0.45  & 1.03& 0.93  & 1.63& 0.23  & 1.52& 0.24  & 1.51& 0.29  \\
Description: \emph{Techniques}      &0.95& 0.89  & 2.05& 0.06  & 1.16& 0.69  & 1.16& 0.73  & 1.50& 0.27  & 2.01& 0.07  \\
 Description: \emph{Enables}      &1.25& 0.51  & \textbf{2.11} & \textbf{0.05*}  & 1.62& 0.18  & 1.42& 0.39  & \textbf{2.20} & \textbf{0.02*}  & 1.98& 0.08  \\
   Description: \emph{Trust}      & 1.27& 0.49  & 1.27& 0.56  & 0.86& 0.69  & 1.69& 0.21  & 1.37& 0.4  & 1.66& 0.21  \\
 Description: \emph{Risk}         &1.65& 0.13  & 2.04& 0.06  & 1.28& 0.5  & 1.48& 0.34  & 1.85& 0.09  & \textbf{2.15} & \textbf{0.05*}  \\
 Description: \emph{Technical}    & 1.54& 0.21  & 1.24& 0.6  & 0.97& 0.93  & 1.48& 0.35  & 0.94& 0.87  & 0.87& 0.75  \\
 \midrule
Internet Score                   & 0.92& 0.44  & 1.09& 0.47  & 1.10& 0.4  & 0.94& 0.61  & 1.03& 0.76  & 1.03& 0.78  \\
Gender: woman                     &0.74& 0.1  & \textbf{0.61} & \textbf{0.02*}  & 0.86& 0.47  & 0.67& 0.07  & \textbf{0.57} & $<$ \textbf{0.01**}  & \textbf{0.65} & \textbf{0.05*}  \\
Race: black                      &0.94& 0.83  & 0.75& 0.37  & 0.88& 0.69  & 0.66& 0.23  & 0.63& 0.13  & 0.77& 0.42  \\
Race: asian                      & 0.75& 0.38  & \textbf{0.16} & $<$ \textbf{0.01**}  & \textbf{0.33} & \textbf{0.02*}  & 0.50& 0.13  & 0.52& 0.09  & \textbf{0.40} & \textbf{0.04*}  \\
Race: hispanic                   &0.76& 0.49  & 1.18& 0.7  & \textbf{2.38} & \textbf{0.02*}  & 0.96& 0.93  & 0.76& 0.49  & 1.55& 0.27  \\
Race: native american               &5.80& 0.08  & 1.57& 0.71  & 1.85& 0.53  & 1.77& 0.63  & 3.09& 0.26  & 5.86& 0.06  \\
Edu: Some College                  & 0.54& 0.08  & 1.18& 0.7  & 1.36& 0.46  & 1.51& 0.32  & 1.94& 0.1  & 1.04& 0.92  \\
Edu: Bachelors+                   &1.54& 0.19  & 1.84& 0.12  & 1.82& 0.13  & 0.75& 0.49  & 1.73& 0.16  & 0.99& 0.97  \\
Income: \$30k-\$50k               &1.66& 0.06  & 1.02& 0.94  & 1.48& 0.19  & \textbf{2.11} & \textbf{0.03*}  & 1.61& 0.1  & 0.97& 0.91  \\
Income: \$50k-\$100k                  & 1.03& 0.92  & 0.81& 0.46  & 1.17& 0.59  & \textbf{2.03} & \textbf{0.03*}  & 1.16& 0.6  & 1.44& 0.2  \\
Income: \$100k-\$200k               & \textbf{0.43} & \textbf{0.02*}  & 0.51& 0.1  & 0.90& 0.79  & 1.83& 0.15  & 0.93& 0.85  & 0.91& 0.8  \\
Income: \$200k+                   & 1.02& 0.97  & 1.01& 0.98  & 1.00& 0.99  & \textbf{6.15} & $<$ \textbf{0.01**}  & 2.65& 0.09  & 1.64& 0.42  \\
  
   \bottomrule
\end{tabular}
\end{table*}




\clearpage


\begin{table*}[ht]
\centering
\caption{Caring by Demographics}
\small
% \label{tab:carebydemo}
\begin{tabular}{lrl|rl|rl|rl|rl|rl} 
  \toprule
  \multicolumn{1}{c|}{\textbf{Variable}}  & \multicolumn{2}{c|}{\textbf{\emph{Exact}}} & \multicolumn{2}{c|}{\textbf{\emph{Hack}}} & \multicolumn{2}{c|}{\textbf{\emph{Law Enforcement}}} & \multicolumn{2}{c|}{\textbf{\emph{Data Analyst}}} & \multicolumn{2}{c|}{\textbf{\emph{Graphs}}} & \multicolumn{2}{c}{\textbf{\emph{Share}}}\\
  \midrule
   & OR & p value & OR  & p value  & OR  & p value & OR  & p value & OR  & p value & OR  & p value  \\ 
  \midrule
% (Intercept) &            0.68 &  0.27  & 1.05 &     0.89    & 0.53 &   0.08   & 0.26 &      $<$ 0.01***  &          0.25 &    $<$ 0.01***   & 0.93 &0.84 \\ 
Salary Scenario        &     1.08 &    0.5    &   0.62 &   $<$ 0.01***    &     0.47   &   $<$ 0.01***  & 0.77 &      0.03*   &    0.93 &      0.57      &   0.63 &   $<$ 0.01*** \\  
Internet Score         &     1.00 &    0.95   &   1.13 &       0.06       &     1.10   &       0.15     & 1.12 &      0.1     &    1.02 &      0.78      &   0.99 &       0.94    \\ 
Age                    &     1.01 &    0.07   &   1.01 &       0.38       &     1.01   &       0.28     & 1.01 &      0.02*   &    1.02 &  $<$ 0.01***   &   1.02 &   $<$ 0.01**  \\ 
Gender: woman          &     0.96 &    0.74   &   0.88 &       0.28       &     0.77   &       0.04*    & 0.89 &      0.32    &    0.98 &      0.86      &   1.04 &       0.76    \\ 
Race: black            &     1.23 &    0.27   &   1.22 &       0.29       &     1.43   &       0.06     & 1.75 &  $<$ 0.01**  &    1.43 &      0.06      &   0.93 &       0.71    \\ 
Race: asian            &     1.17 &    0.46   &   2.28 &   $<$ 0.01***    &     1.98   &   $<$ 0.01**   & 1.71 &      0.01*   &    1.79 &      0.01**    &   2.35 &   $<$ 0.01*** \\ 
Race: hispanic         &     0.85 &    0.5    &   1.27 &       0.31       &     1.51   &       0.08     & 1.26 &      0.32    &    1.22 &      0.4       &   0.93 &       0.75    \\ 
Race: native american  &     4.46 &    0.02*  &   1.42 &       0.48       &     1.99   &       0.17     & 2.05 &      0.15    &    1.67 &      0.3       &   1.90 &       0.24    \\ 
Edu: Some College      &     0.80 &    0.35   &   1.09 &       0.7        &     1.27   &       0.33     & 1.38 &      0.18    &    1.01 &      0.96      &   1.37 &       0.21    \\ 
Edu: Bachelors+        &     1.18 &    0.45   &   0.79 &       0.28       &     1.03   &       0.91     & 1.24 &      0.34    &    0.96 &      0.84      &   0.50 &   $<$ 0.01**  \\ 
Income: \$30k-\$50k    &     1.15 &    0.44   &   0.83 &       0.33       &     1.02   &       0.93     & 1.16 &      0.43    &    0.99 &      0.97      &   1.15 &       0.45    \\ 
Income: \$50k-\$100k   &     1.05 &    0.8    &   0.84 &       0.32       &     0.93   &       0.68     & 1.16 &      0.4     &    1.20 &      0.31      &   1.53 &       0.02*   \\ 
Income: \$100k-\$200k  &     1.09 &    0.69   &   0.99 &       0.95       &     1.05   &       0.82     & 1.18 &      0.45    &    1.81 &      0.01**    &   2.83 &   $<$ 0.01*** \\ 
Income: \$200k+        &     1.06 &    0.9    &   0.62 &       0.29       &     1.15   &       0.77     & 1.08 &      0.86    &    0.81 &      0.66      &   3.82 &       0.01**  \\     
   \bottomrule
\end{tabular}
\end{table*}

\clearpage


\begin{table}[ht]
\centering
\caption{Setting Expectations Explicitly}
\small
\label{tab:explicitexpectationscombined}
\begin{tabular}{lrll}
  \hline
 Variable & Odds Ratio & CI & p value \\ 
  \hline
 (Intercept) & 0.41 & [0.22, 0.75] & $<$ 0.01** \\ 
 Condition: Differential Privacy & 1.27 & [0.9, 1.79] & 0.17 \\ 
 Salary Scenario & \textbf{1.62} & \textbf{[1.27, 2.07]} & $<$ \textbf{0.01***} \\ 
 Internet Score & 1.10 & [0.95, 1.26] & 0.2 \\ 
 Gender: woman & 0.73 & [0.57, 0.93] & 0.01* \\ 
 Race: black & 0.91 & [0.63, 1.33] & 0.62 \\ 
 Race: asian & \textbf{0.37} & \textbf{[0.23, 0.59]} & $<$ \textbf{0.01***} \\ 
 Race: hispanic & 0.68 & [0.42, 1.08] & 0.1 \\ 
 Race: native american & 1.36 & [0.45, 4.3] & 0.59 \\ 
 Edu: Some College & 1.22 & [0.77, 1.94] & 0.4 \\ 
 Edu: Bachelors+ & \textbf{1.89} & \textbf{[1.23, 2.92]} & $<$ \textbf{0.01**} \\ 
 Income: \$30k-\$50k   & \textbf{1.65} & \textbf{[1.14, 2.39]} & \textbf{0.01**} \\ 
 Income: \$50k-\$100k   & 1.50 & [1.06, 2.13] & 0.02* \\ 
 Income: \$100k-\$200k  & 1.46 & [0.92, 2.33] & 0.11 \\ 
 Income: \$200k+        & 2.15 & [0.9, 5.58] & 0.1 \\ 
   \hline
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Share With Nameless Privacy Protections}
\small
\label{tab:sharewithdp}
\begin{tabular}{lrll}
  \hline
 Variable & Odds Ratio & CI & p value \\ 
  \hline
Expectation \emph{Exact}: No Risk & 1.61 & [1.12, 2.32] & 0.01* \\ 
Expectation \emph{Exact}: Low Risk & 1.49 & [1.04, 2.16] & 0.03* \\ 
Expectation \emph{Exact}: High Risk & 1.01 & [0.69, 1.47] & 0.97 \\ 
Expectation \emph{Hack}: No Risk & 2.05 & [1.41, 2.98] & $<$ 0.01*** \\ 
Expectation \emph{Hack}: Low Risk & 1.27 & [0.87, 1.84] & 0.22 \\ 
Expectation \emph{Hack}: High Risk & 0.58 & [0.39, 0.86] & 0.01** \\ 
Expectation \emph{Law Enforcement}: No Risk & 1.37 & [0.91, 2.07] & 0.13 \\ 
Expectation \emph{Law Enforcement}: Low Risk & 0.60 & [0.39, 0.91] & 0.02* \\ 
Expectation \emph{Law Enforcement}: High Risk & 0.62 & [0.41, 0.94] & 0.03* \\ 
Expectation \emph{Data Analyst}: No Risk & 0.92 & [0.61, 1.39] & 0.7 \\ 
Expectation \emph{Data Analyst}: Low Risk & 0.60 & [0.39, 0.9] & 0.02* \\ 
Expectation \emph{Data Analyst}: High Risk & 0.74 & [0.49, 1.12] & 0.16 \\ 
Expectation \emph{Graph}: No Risk & 0.66 & [0.43, 0.99] & 0.05* \\ 
Expectation \emph{Graph}: Low Risk & 0.75 & [0.49, 1.14] & 0.18 \\ 
Expectation \emph{Graph}: High Risk & 0.44 & [0.28, 0.68] & $<$ 0.01*** \\ 
Expectation \emph{Share}: No Risk & 0.64 & [0.45, 0.92] & 0.02* \\ 
Expectation \emph{Share}: Low Risk & 0.40 & [0.28, 0.59] & $<$ 0.01*** \\ 
Expectation \emph{Share}: High Risk & 0.27 & [0.19, 0.4] & $<$ 0.01*** \\ 
\midrule
Salary Scenario & 1.10 & [0.84, 1.43] & 0.49 \\ 
Internet Score & 1.01 & [0.88, 1.17] & 0.85 \\ 
Gender: woman & 0.80 & [0.62, 1.04] & 0.1 \\ 
Race: black & 1.09 & [0.73, 1.63] & 0.66 \\ 
Race: asian & 0.44 & [0.27, 0.72] & $<$ 0.01** \\ 
Race: hispanic & 2.15 & [1.3, 3.63] & $<$ 0.01** \\ 
Race: native american & 1.90 & [0.7, 5.39] & 0.21 \\ 
Edu: Some College & 0.63 & [0.38, 1.03] & 0.07 \\ 
Edu: Bachelors+ & 1.16 & [0.73, 1.85] & 0.54 \\ 
Income: \$30k-\$50k       & 1.22 & [0.82, 1.81] & 0.33 \\ 
Income: \$50k-\$100k       & 1.13 & [0.77, 1.64] & 0.54 \\ 
Income: \$100k-\$200k       & 1.06 & [0.66, 1.71] & 0.81 \\ 
Income: \$200k+           & 0.53 & [0.19, 1.41] & 0.21 \\ 
Age & 1.00 & [0.98, 1.01] & 0.44 \\ 
   \hline
\end{tabular}
\end{table}


\begin{table*}[ht]
\centering
\caption{Effects on Sharing when setting explicit expectations -- split out}
\small
% \label{tab:carebydemo}
\begin{tabular}{lrl|rl|rl|rl|rl|rl} 
  \toprule
  \multicolumn{1}{c|}{\textbf{Variable}}  & \multicolumn{2}{c|}{\textbf{\emph{Exact}}} & \multicolumn{2}{c|}{\textbf{\emph{Hack}}} & \multicolumn{2}{c|}{\textbf{\emph{Law Enforcement}}} & \multicolumn{2}{c|}{\textbf{\emph{Data Analyst}}} & \multicolumn{2}{c|}{\textbf{\emph{Graphs}}} & \multicolumn{2}{c}{\textbf{\emph{Share}}}\\
  \midrule
   & OR & p value & OR  & p value  & OR  & p value & OR  & p value & OR  & p value & OR  & p value  \\ 
  \midrule
Low Risk &                     1.78 &                   0.01** & 2.05 &        $<$ 0.01** & 0.91 &       0.72 & 0.85 &      0.49 & 1.57 &      0.07  & 1.34 &      0.15 \\ 
No Risk &                      1.78 &                   $<$ 0.01** & 3.10 &        $<$ 0.01*** & 2.40 &       $<$ 0.01*** & 1.12 &      0.62 & 1.50 &        0.11  & 2.24 &        $<$ 0.01*** \\ 
\midrule
Salary Scenario &                      1.23 &                     0.2 & 1.50 &        0.02* & 1.51 &   0.05* & 1.49 &      0.04* & 1.23 &        0.31  & 1.07 &        0.68 \\ 
Internet Score &                      0.97 &                   0.73 & 1.01 &          0.89 & 1.03 &         0.8 & 1.30 &        0.02* & 1.02 &        0.88  & 1.00 &      0.98 \\ 
Gender: woman &                     0.80 &                   0.18 & 0.85 &        0.38 & 0.80 &       0.3 & 1.04 &      0.84 & 0.95 &      0.8  & 0.88 &      0.43 \\ 
Race: black &                     1.22 &                   0.43 & 1.15 &        0.6 & 1.91 &       0.03* & 1.54 &      0.11 & 1.10 &      0.74  & 0.91 &      0.73 \\ 
Race: asian &                     0.39 &                   $<$ 0.01** & 0.36 &        $<$ 0.01*** & 0.23 &       $<$ 0.01*** & 0.42 &      0.01* & 0.42 &      0.02*  & 0.32 &      $<$ 0.01*** \\ 
Race: hispanic &                      1.73 &                   0.11 & 2.39 &        0.01** & 2.13 &       0.04* & 1.80 &    0.09 & 2.52 &        0.01*  & 1.92 &        0.04* \\ 
Race: native american &                      1.81 &                   0.27 & 1.91 &        0.31 & 2.13 &       0.26 & 2.02 &    0.27 & 3.41 &        0.08  & 2.59 &        0.1 \\ 
Edu: Some College &                      0.53 &                     0.06 & 0.56 &          0.07 & 0.53 &         0.12 & 0.46 &        0.06 & 0.42 &        0.04*  & 0.61 &      0.11 \\ 
Edu: Bachelors+ &                     1.50 &                   0.18 & 0.97 &        0.93 & 1.37 &       0.41 & 0.97 &      0.93 & 1.23 &      0.58  & 0.81 &        0.48 \\ 
Income: \$30k-\$50k    &            1.18 &                   0.53 & 1.18 &        0.53 & 0.95 &       0.88 & 0.98 &      0.95 & 1.23 &      0.53  & 1.05 &        0.86 \\ 
Income: \$50k-\$100k   &              0.80 &                   0.35 & 1.17 &          0.52 & 0.90 &       0.72 & 0.93 &        0.81 & 1.06 &        0.84  & 0.87 &      0.58 \\ 
Income: \$100k-\$200k  &              0.69 &                   0.23 & 1.09 &        0.77 & 0.84 &       0.63 & 1.72 &      0.12 & 1.42 &      0.33  & 1.13 &        0.67 \\ 
Income: \$200k+        &            0.40 &                     0.15 & 0.85 &          0.82 & 0.73 &         0.69 & 0.83 &        0.81 & 1.36 &        0.72  & 0.71 &      0.56 \\ 
Age &                      0.99 &                 0.13 & 0.99 &      0.11 & 0.99 &         0.49 & 0.99 &        0.2 & 0.98 &    0.11  & 0.99 &    0.07 \\   
   \bottomrule
\end{tabular}
\end{table*}



\begin{table*}[ht]
\centering
\caption{More Correct by Definition}
\small
\label{tab:correctlocalcentral}
\begin{tabular}{lrl|rl|rl|rl|rl|rl} 
  \toprule
  \multicolumn{13}{c}{\textbf{Local Differential Privacy Model}} \\
  \midrule
  \multicolumn{1}{c}{\textbf{Variable}}  & \multicolumn{2}{|c}{\textbf{\emph{Exact}}} & \multicolumn{2}{|c}{\textbf{\emph{Hack}}} & \multicolumn{2}{|c}{\textbf{\emph{Law Enforcement}}} & \multicolumn{2}{|c}{\textbf{\emph{Data Analyst}}} & \multicolumn{2}{|c}{\textbf{\emph{Graphs}}} & \multicolumn{2}{|c}{\textbf{\emph{Share}}}\\
  \midrule
   & OR & p value & OR  & p value  & OR  & p value & OR  & p value & OR  & p value & OR  & p value  \\ 
  \midrule
Description: \emph{Unsubstantial}  & 0.79 & 0.3 & 0.70 & 0.11 & 0.79 & 0.3 & 0.66 & 0.08 & \textbf{0.63} & \textbf{0.04*} & 0.72 & 0.16 \\ 
Description: \emph{Techniques}  & 0.90 & 0.64 & \textbf{0.60} & \textbf{0.02*} & \textbf{0.63} & \textbf{0.03*} & \textbf{0.60} & \textbf{0.03*} & \textbf{0.51} & $<$ \textbf{0.01**} & \textbf{0.40} & $<$ \textbf{0.01***} \\ 
Description: \emph{Enables}   & 0.79 & 0.29 & 0.85 & 0.47 & 0.86 & 0.5 & 0.64 & 0.06 & \textbf{0.60} & \textbf{0.02*} & \textbf{0.61} & \textbf{0.03*} \\ 
Description: \emph{Trust}   & 0.84 & 0.43 & 0.76 & 0.22 & 0.89 & 0.62 & 0.87 & 0.55 & 0.77 & 0.24 & 0.81 & 0.38 \\ 
Description: \emph{Risk}   & 0.88 & 0.56 & \textbf{0.41} & $<$ \textbf{0.01***} & \textbf{0.47} & $<$ \textbf{0.01***} & \textbf{0.47} & $<$ \textbf{0.01**} & \textbf{0.46} & $<$ \textbf{0.01***} & \textbf{0.47} & $<$ \textbf{0.01***} \\ 
Description: \emph{Technical}   & 0.92 & 0.72 & \textbf{0.63} & \textbf{0.04*} & 0.85 & 0.46 & \textbf{0.47} & $<$ \textbf{0.01**} & \textbf{0.58} & \textbf{0.01*} & \textbf{0.55} & \textbf{0.01**} \\ 
\midrule
Salary Scenario       & 1.15 & 0.25 & 0.93 & 0.57 & \textbf{1.44} & $<$ \textbf{0.01**} & \textbf{1.27} & \textbf{0.05*} & 0.92 & 0.49 & 0.85 & 0.19 \\ 
Internet Score        & 0.94 & 0.39 & \textbf{0.81} & $<$ \textbf{0.01**} & 0.83 & \textbf{0.01**} & 1.03 & 0.63 & 0.94 & 0.34 & 0.98 & 0.81 \\ 
\toprule
 \multicolumn{13}{c}{\textbf{Central Differential Privacy Model}} \\
\midrule
\multicolumn{1}{c}{\textbf{Variable}}  & \multicolumn{2}{|c}{\textbf{\emph{Exact}}} & \multicolumn{2}{|c}{\textbf{\emph{Hack}}} & \multicolumn{2}{|c}{\textbf{\emph{Law Enforcement}}} & \multicolumn{2}{|c}{\textbf{\emph{Data Analyst}}} & \multicolumn{2}{|c}{\textbf{\emph{Graphs}}} & \multicolumn{2}{|c}{\textbf{\emph{Share}}}\\
  \midrule
Description: \emph{Unsubstantial}& 0.79 & 0.3 & \textbf{1.94} & \textbf{0.01*} & 1.10 & 0.72 & 1.71 & 0.1 & 0.63 & \textbf{0.04*} & 1.68 & 0.06 \\ 
Description: \emph{Techniques} &0.90 & 0.64 & \textbf{1.96} & \textbf{0.01*} & 1.21 & 0.47 & \textbf{2.40} & $<$ \textbf{0.01**} & \textbf{0.51} & $<$ \textbf{0.01**} & \textbf{2.22} & $<$ \textbf{0.01**} \\ 
Description: \emph{Enables} &0.79 & 0.29 & 1.60 & 0.08 & 1.05 & 0.84 & \textbf{2.06} & \textbf{0.02*} & \textbf{0.60} & \textbf{0.02*} & 1.69 & 0.05 \\ 
Description: \emph{Trust} & 0.84 & 0.43 & \textbf{1.86} & \textbf{0.02*} & 1.04 & 0.89 & \textbf{1.99} & \textbf{0.03*} & 0.77 & 0.24 & 1.19 & 0.55 \\ 
Description: \emph{Risk} & 0.88 & 0.56 & \textbf{2.58} & $<$ \textbf{0.01***} & \textbf{1.86} & \textbf{0.01*} & \textbf{2.46} & $<$ \textbf{0.01**} & \textbf{0.46} & $<$ \textbf{0.01***} & \textbf{2.27} & $<$ \textbf{0.01**} \\ 
Description: \emph{Technical} &0.92 & 0.72 & 1.56 & 0.1 & 1.02 & 0.95 & \textbf{2.30} & \textbf{0.01**} & \textbf{0.58} & \textbf{0.01*} & \textbf{1.90} & \textbf{0.02*} \\ 
\midrule
Salary Scenario & 1.15 & 0.25 & \textbf{1.32} & \textbf{0.04*}& 0.80 & 0.11 & 0.75 & 0.06 & 0.92 & 0.49 & 1.14 & 0.31 \\
Internet Score & 0.94 & 0.39 & \textbf{1.17} & \textbf{0.04*} & \textbf{1.25} & \textbf{0.01**} & 1.05 & 0.54 & 0.94 & 0.34 & 1.01 & 0.85 \\ 

  
   \bottomrule
\end{tabular}
\end{table*}

 

==> tpdp_background.tex <==
\medskip \noindent
\textbf{Background and Related Work} A large body of prior work has examined how best to explain privacy to end users~\cite{mcdonald2009comparative,spiekermann2008engineering,earp2005examining,jensen2004privacy,senarath2017designing, kelley2009nutrition, motti2016towards, egelman2015thing, cranor2006they, sadeh2013usable, schaub2017designing}. Despite this large body of prior work on privacy communications and the increasing importance of DP, only two pieces of prior work have focused on communicating with users about DP. Bullek et. al. \cite{bullek2017towards} study how users understand privacy parameters in randomized response, a specific local DP technique. Our work focuses more broadly on how the information disclosures against which DP can protect influence user's willingness to share, and on how descriptions of DP influence expectations for those information disclosures.  Xiong et al. \cite{SP:XWLJ20} study how informing users that their information is protected with DP influences their willingness to share different types of information. They study this question in the context of an app that collects medically relevant information. They found that promising users DP makes them more willing to share their information, but users struggled to understand descriptions of DP. Our work builds upon this prior work to more deeply explore (RQ1) which information sharing implications are most concerning to users, and thus should be emphasized when describing DP, (RQ2) how these implications themselves influence users willingness to share information, and (RQ3) how existing, in-the-wild descriptions of DP set their expectations about these information sharing implications. Additionally, we seek to replicate their results through (RQ4), in which we examine how different descriptions of DP themselves influence users willingness to share information. 

% In addition to primarily focusing on different research questions our work methodologically differs from the work of Xiong et al. in two ways. First, we derive the descriptions of DP we use as stimuli from a systematic review of 76 in-the-wild descriptions of DP (see Section~\ref{sec:surveytwo}). In contrast, in two of their three experiments Xiong et al. use DP descriptions that were created to explain the definition and/or different aspects ({\em e.g.}, data perturbation) of DP to users\footnote{The most closely related definition to our work is the DP with implications description: ``To respect your personal information privacy and ensure best user experience, the data shared with the app will be processed via the differential privacy (DP) technique. That is, the app company will store your data but only use the aggregated statistics with modification so that your personal
% information cannot be learned. However, your personal information may be leaked if the company’s database is compromised.''}; more similar to our approach, in their third experiment they use the descriptions from four companies that use DP, in addition to their created descriptions. Second, and relatedly, 
% Xiong et al. test that respondents correctly understand the implications of DP based on the description they were shown, before respondents are shown additional survey questions about their willingness to share information. Respondents who did not correctly answer the understanding question(s) were presented with the DP description a second time; if they again did not understand the description, they were excluded from the study. Their results thus have important implications about how users can be educated about DP. On the other hand, this methodology does not offer insight into how users' privacy expectations or willingness to share information might be influenced by encountering descriptions of DP in the wild, rather than in a laboratory setting. As further discussed in Section~\ref{sec:discussion}, the results of our replication study (RQ4) significantly differ from those of Xiong et al. likely due to the methodological differences in our approaches.

==> tpdp_intro.tex <==
\vspace{-1em}
\section{Introduction}

% Differential privacy (DP) is a mathematically rigorous definition of privacy that has gained popularity since its formalization in 2006 \cite{TCC:DMNS06}. DP facilitates the computation of aggregate statistics about a dataset while placing a formal bound on the amount of information that these statistics can disclose about individual data points within the dataset. Guaranteeing DP generally requires injecting carefully calibrated noise that hides individual datapoints while preserving aggregate level insights.

Differential Privacy \cite{TCC:DMNS06} (DP) has become a leading technique used to meet the increasing consumer demand for digital privacy \cite{pewsurvey}. In the last few years, several companies have  deployed DP. For instance, Apple uses DP to gather aggregate statistics on Emoji usage, which it uses to order Emojis for users \cite{appledp, appledpshort}. Uber uses DP to prevent data analysts within the company from stalking customers \cite{uberdpconference,uberdpgithub}, and Google uses DP to crowd-source statistics from Google Chrome crash reports \cite{CCS:ErlPihKor14}. The U.S. government has also begun to use DP for the 2020 decennial census \cite{censusdp}, meaning that nearly every person in the United States will have private data protected by DP. Following in the footsteps of these earlier adopters, more companies have already announced their intentions to integrate differentially private techniques into their systems, {\em e.g.} \cite{facebookone,facebooktwo}. As a result, DP is becoming an increasingly consumer-relevant technology. Yet, little is known about whether end users value the protections offered by DP.

While DP is mathematically elegant and computationally efficient, it can be difficult to understand. Not only is DP typically defined mathematically, but the privacy protections provided by DP are not absolute and require contextualization \cite{Dwork08}. DP does not provide binary privacy ({\em i.e.} private or not private), but instead provides a statistical privacy controlled by unitless system parameters that are difficult to interpret ({\em i.e.}, the parameters $\epsilon$ and $\delta$ control the maximum amount of information that can leak about any individual entry in the dataset) \cite{TCC:DMNS06}. %Additionally, DP can be deployed in different security models, and the choice of model has a significant impact on the types of adversarial behavior the system can tolerate.  In the \emph{local} model, users randomly perturb their information (with the help of the collection mechanism, {\em e.g.,} their device) before sending it to a central entity in charge of analysis, called the curator \cite{KLNRS11}.  In the \emph{central} model, users share their sensitive information directly, and the curator is trusted to perturb any analysis results that are released \cite{DR14}. 

\smallskip \noindent
\textbf{Differential Privacy from the user's perspective.} The existing DP literature focuses on techniques for achieving DP\elissa{these cites aren't happy?} \cite{TCC:DMNS06,DR14,FOCS:McSTal07, FOCS:HarRot10,STOC:DNRRV09,KLNRS11,DFH+15}, with a small but growing body of work on legal and ethical implications of DP \cite{nissim2018privacy,cummings2018role, oberski2020differential, cohen2020towards}. Notably absent, however, is the voice of the end user, whose information may eventually be protected by DP and may benefit from its deployment~\cite{benthall2017contextual}. Do users care about the information disclosures against which DP protects? Do users understand how DP protects them, and if so, do those protections influence their comfort with sharing information? As differentially private systems proliferate, it is increasingly important to answer such questions and understand DP from the \emph{user's} perspective.
%

% While a limited body of prior work has sought to understand how training users to understand DP influences willingness to share \cite{SP:XWLJ20, bullek2017towards,DCHL21}, we aim to answer broader questions regarding:  \begin{enumerate*}[(i)]
%     \item whether DP meets users' existing privacy needs,
%     \item what expectations a potential user might have of a differentially private system, and
%     \item whether existing, in-the-wild, descriptions of DP accurately set user expectations.
% \end{enumerate*}  

As a privacy-enhancing technology, DP is designed to prevent the unwanted information disclosure of user information to certain entities. However, it is not clear that these protections are meaningful to potential users. Additionally, it is not clear if DP provides the level of protection that potential users might hope.

Thus, in this work, we ask the following research questions:

\begin{enumerate}

  \item[\textbf{(RQ1)}] Do potential users care about protecting their information against disclosure to the entities against which differentially private systems can protect? 
  \item[\textbf{(RQ2)}] Are potential users more willing to share their information when they have increased confidence such information disclosures will not occur?
  \item[\textbf{(RQ3)}] Do potential users expect differentially private systems to protect their information against disclosure? How does the way in which differential privacy is described impact their expectations?
  \item[\textbf{(RQ4)}]  Are potential users more willing to share their information when their information will be protected with differential privacy?  How does the way in which differential privacy is described impact sharing?
   
\end{enumerate}
We conduct two surveys with a total of $2,424$ respondents to answer our research questions. We use vignette-based surveys to elicit respondents' intended behavior as such surveys have been found to well-approximate real world behavior~\cite{hainmueller2015validating}. 

To address RQ1 and RQ2, we present each respondent with one of two information-sharing scenarios (sharing information with a salary transparency initiative or sharing medical records with a research initiative) and query respondents' privacy concerns. We then set their privacy expectations for those concerns (e.g., how likely information is to be leaked to a particular entity) and query if they would be willing to share their private information. Using the results of this survey, we examine how respondents' privacy concerns align with the protections offered by DP.

To address RQ3 and RQ4, we again present each respondent with one of the two information-sharing scenarios. We additionally tell respondents that their information will be protected by DP, as described by one of six descriptions.\footnote{We also maintain a control group of participants who are not told that their information is protected.} We then query respondents' privacy expectations for these scenarios (e.g., whether their information could leak to various entities) and whether they would be willing to share their information. Using the results of this survey, we interrogate how accurately and effectively existing descriptions of DP set user expectations.

There is no ``standard'' deployment of DP, nor is there a ``normal'' way to describe its guarantees. In order to define representative descriptions of DP to present to our participants, we systematically collected over 70 descriptions of DP written by companies, government agencies, news outlets, and academic publications. Through affinity diagramming qualitative analysis~\cite{beyer1999contextual}, we identify six main themes present in these descriptions
and compose a representative description for each theme that we showed to respondents.

By describing DP as a potential user would encounter it in the wild, we gain a better understanding of how potential users are likely to respond to DP in practice. The nuances innate in DP make it easy for a prospective user to misunderstand what they are being promised. As such, a user seeking to choose the right privacy preserving system may find it difficult to make an informed choice. Getting this wrong can have real world consequences: DP may be insufficient to protect a user's information against the types of threats about which they are concerned.

% \smallskip \noindent
% \textbf{Summary of Findings.} We find that users generally do care about the kinds of information disclosure against which DP can protect against \textbf{(RQ1)} and are more willingness to share their private information when the risk of information disclosure to certain entities, specifically those for which disclosure would represent an inappropriate information flow~\cite{nissenbaum2004privacy}, was not possible \textbf{(RQ1)}. Surprisingly, however, we found that informing users that a system was differentially private did \emph{not} raise potential user's willingness to share information \textbf{(RQ2)}, no matter which description of DP was presented to the respondent. This contradicts findings in \cite{SP:XWLJ20}, which indicated that DP did increase willingness to share information. We believe this difference indicates that the manner in which DP is described, and the context in which it is used, may have significant impact on user's understanding and behavior.

% Although descriptions of DP did not increase potential user's willingness to share information, we did find that different descriptions of DP did raise respondent's concrete privacy expectations around information disclosure \textbf{(RQ3)}. This effect, however, varied by description. That is, different descriptions of DP raise expectations for different kinds of information disclosure. These expectations, in turn, raised respondent's willingness to share information.

% As a whole, our results suggest a framework for understanding how descriptions of DP interact with user's concrete privacy expectations and willingness to share information: individual users may care about different kinds of information disclosure. When DP is described to a potential user, it is likely to raise \emph{some} of their expectations, but not necessarily the ones that significantly influence that user's decision. Put another way, the common methods for describing DP are not precise communication mechanisms and may raise user's privacy expectations in unintended ways. This lesson is especially important for central DP systems, which protect user's privacy against fewer kinds of malicious behavior. In this case, using imprecise descriptions of DP my inappropriately raise user's expectations, giving users a false sense of security.

\smallskip \noindent
\textbf{Summary of Findings.} We find that users care about the kinds of information disclosure against which DP can protect (RQ1) and are more willing to share their private information when the risk of information disclosure to certain entities, specifically those for which disclosure would represent an inappropriate information flow~\cite{nissenbaum2004privacy}, is not possible (RQ2).

Further, we find that descriptions of DP raise respondent's concrete privacy expectations around information disclosure (RQ3). This effect, however, varies by how DP is described: different descriptions of DP raise expectations for different kinds of information disclosure. These expectations, in turn, raise respondent's willingness to share information. However, informing respondents that a system was differentially private did \emph{not} raise potential user's willingness to share information, no matter which description of DP was presented to the respondent (RQ4). %This contradicts findings in \cite{SP:XWLJ20}, which indicated that DP did increase willingness to share information. We believe this difference indicates that the manner in which DP is described, and the context in which it is used, may have significant impact on user's understanding and behavior.

Taken together, our findings suggest that while (1) respondents do care about the information disclosures against which DP can protect; (2) the likelihood of those disclosures influences respondent's willingness to share; and (3) different in-the-wild descriptions of DP influence respondents perception of the likelihood of those disclosures. However, (4) simply being shown a randomly selected, in-the-wild description of DP does not increase willingness to share.  These results, at first glance, appear to be in tension.

On deeper analysis, however, these findings suggest the presence of a misalignment between the information disclosures about which users care and the information disclosures that descriptions of DP address. The probability that a given respondent was (a) shown a description that related to the information disclosures about which they care, and (b) that description influenced enough of their perceptions is likely low. 

Synthesizing these findings, we posit a novel framework for understanding how end users reason about sharing their data under DP protections. % that rectifies this seeming contradiction:  
Our framework --- and the findings that informed it --- offer concrete directions for reformulating DP descriptions to accurately and effectively set user's privacy expectations and increase their comfort when using differentially private systems.  Users must either be trained to carefully understand descriptions (as done in \cite{SP:XWLJ20}) or descriptions should be reformulated to directly communicate how they address the information flows that concern users (e.g., via privacy nutrition-labels~\cite{kelley2009nutrition}). If DP descriptions can be effectively reformulated, our results suggest that users may be significantly more comfortable sharing their information when given differentially private protections. 
%
% \smallskip \noindent
% \textbf{Contributions}. In summary, our contributions are as follows
% \begin{itemize}[--]
%   \item \textbf{Deepening our Understanding of User's Privacy Concerns and Willingness to Share.}

%   \item \textbf{Systematization of the ways DP in the Wild.}
    
%   \item \textbf{Understanding how users .}

%   \item \textbf{Framework for Understanding How Descriptions of DP Impact Willingness to Share.}
% \end{itemize}
%\elissa{this paper talks about how CI has NOT been applied to DP: \url{https://www.cs.ru.nl/~jhh/ans/2018/lit/j3-botnets/Contextual\%20Integrity\%20Through\%20the\%20Lense\%20of\%20CS.pdf}}

==> tpdp_methods.tex <==
\section{Summary of Methods}\label{sec:methods}
To answer our research questions, we ran two vignette (scenario) surveys~\cite{hainmueller2015validating} ($n = 2424$ total) via Amazon Mechanical Turk, one to address RQ1 and RQ2 and the other to address RQ3 and RQ4. In both our surveys, we use the same two scenarios, which focus on two different potential use cases for DP: protecting people's salaries and protecting people's medical histories. The full wording of these scenarios, along with the full questionnaires, are available in the full version of this work.  MTurk has been shown to be representative of American privacy preferences for Americans aged 18-50 who have at least some college education~\cite{SP:RedKroMaz19}.  Our procedures were approved by our institutions' ethics review boards.

\medskip \noindent
\textbf{Survey One: (RQ1) and (RQ2)} In our first survey, we asked respondents about their willingness to share their information if there was a risk of information disclosure to particular entities.  Namely, for each of the following information disclosures, we asked if the respondent \emph{cared} about disclosure to the entity: \begin{itemize*}
 \item[\emph{(Hack)}] Could a criminal organization or foreign government access the respondent's information by hacking the organization holding the information?;
 \item[\emph{(Law Enforcement)}] Could a law enforcement organization access the respondent's information with a court-issued warrant?;
 \item[\emph{(\exactexpectationname)}] Could the organization collecting the information (or their representative) access the respondent's information?;
 \item[\emph{(Data Analyst)}] Could a data analyst working within the organization access the respondent's information?;
 \item[\emph{(Graphs)}] Could graphs or informational charts created by the organization be used to learn the respondent's information?; and
 \item[\emph{(Share)}] Could the collected information be shared with another organization such that the other organization could access the respondent's information?
\end{itemize*} If the responded indicated that they did care, the respondent was told that there was either no risk of disclosure, a small risk of disclosure, or a large risk of disclosure (selected at random).  Finally, we asked if the respondent would be willing to share their information under these conditions.

\medskip \noindent
\textbf{Survey Two: (RQ3) and (RQ4)} We start by gathering 76 in-the-wild  descriptions of differentially privacy. through affinity diagramming~\cite{beyer1999contextual}, the research team identified six main themes in these descriptions (names in bold): \begin{enumerate*}
  \item[\textbf{(Unsubstantial)}] claims that DP is the best notion of privacy;
  \item[\textbf{(Techniques)}] explanations that briefly summarize the methods used to create differentially private summary statistics, usually focusing on statistical noise;
  \item[\textbf{(Enables)}] statements that attempt to capture the types of applications that DP makes possible;
  \item[\textbf{(Trust)}] descriptions that focus on the well known organizations and companies that have recently started using DP;
  \item[\textbf{(Risk)}] statements that highlight the data-privacy risks that an individual incurs when allowing their information to be part of a differentially private system; and 
  \item[\textbf{(Technical)}] highly technical explanations using dense, mathematical language.
\end{enumerate*}  Using these themes, we synthesized representative descriptions for each theme to use in our second survey.

% \input{descriptionstable}
In survey two, the vignette scenario was followed by "To reduce the intrusion into personal privacy, the [organization] will use a technique called differential privacy. [differential privacy description]," where the description presented was sampled with equal weight from the representative descriptions. 
Respondents were then asked the following questions: First, they were asked if they would be willing to share their data. Next, each respondent was asked to share their concrete privacy expectations by reporting whether they believed the expectations described in the Survey One summary (e.g., ``A criminal or foreign government that hacks the transparency initiative could learn my salary and job title.'') were true or false.

% We present detailed overviews of each survey in \cref{sec:surveyone} and \cref{sec:surveytwo} respectively.  Similarly, we present our findings from each survey in \cref{sec:resultsbranch34} and \cref{sec:resultsbranch12} respectively.  Our full survey instruments can be found in \cref{apx:surveys}. We also present demographic information for our survey respondents in \cref{tab:surveydemographics}, also located in the appendix. Our procedures were approved by our institution's ethics review board.

% \input{branch34}

% \input{branch12}

% \subsection{Limitations}
% As in all user studies, our study is subject to multiple possible biases. The first is sampling bias. We sample our respondents using MTurk. While prior work shows that MTurk is reasonably representative of the privacy attitudes and experiences of Americans aged 18-50 who have some college education ~\cite{SP:RedKroMaz19}, our sample does not capture the experiences of all Americans, especially those older and less educated. Our results should be interpreted in this context. Second, we may have introduced reporting biases through our question design. While we aimed to follow best practices --- using cognitive interviews to validate our questionnaire, and offering ``other'' and ``I don't know'' response options~\cite{redmiles2017summary} --- respondents may still have mis-reported or failed to report their true perceptions or preferences. Third, while we took steps to improve external validity --- sourcing experimental stimuli by rigorously collecting and coalescing in-the-wild DP descriptions and using a vignette survey --- our study may have failed to appropriately reflect real-world conditions.

% \input{scenariosexpectationstable}

==> tpdp_resultsanddiscussion.tex <==
\begin{figure*}[t]
	\centering
	\resizebox{\textwidth}{!}{
		\begin{tikzpicture}
		
		\node[anchor=west] at (-13,6) {Legend:};
 \node[circle,draw,fill=red!40] at (-12.5, 5.5) {};
 \node[circle,draw,fill=orange!40] at (-12.5, 5) {};
 \node[circle,draw,fill=yellow!40] at (-12.5, 4.5) {};
 \node[circle,draw,fill=green!40] at (-12.5, 4) {};
 \node[circle,draw,fill=blue!40] at (-12.5, 3.5) {};
 \node[circle,draw,fill=pink!40] at (-12.5, 3) {};
 
 \node[anchor=west] at (-12.25, 5.5) {Hack};
 \node[anchor=west] at (-12.25, 5) {Law Enforcement};
 \node[anchor=west] at (-12.25, 4.5) {\exactexpectationname};
 \node[anchor=west] at (-12.25, 4) {Data Analyst};
 \node[anchor=west] at (-12.25, 3.5) {Graphs};
 \node[anchor=west] at (-12.25, 3) {Share};

		
% 		\node at (-12,-1) {Information Disclosure Risks:};
% Left

 \node[alice,minimum size=1cm] at (-10,.5) {};
 \node[] at (-6,.5) {Description: \emph{Enables}};
 
 \node at (-10,-.5) {User Concerns:};
 \node[circle,draw,fill=pink!40] at (-9.5, -1) {};
 \node[circle,draw,fill=orange!40] at (-10, -1) {};
 \node[circle,draw,fill=red!40] at (-10.5, -1) {};

 \node at (-6,-.5) {Description Effects:};
 \node[circle,draw,fill=green!40] at (-6.25, -1) {};
 \node[circle,draw,fill=blue!40] at (-5.75, -1) {};

 \draw [->] (-10,1.25) -- (-9,2.125);
 
 \draw [->] (-6,1.25) -- (-7,2.125);
	 
 \node[circle,draw,minimum size=70] at (-7.5, 3.5) {};
 \node[circle,draw,minimum size=70] at (-8.5, 3.5) {};
 \node at (-8,1.75) {No Overlap};
 

 \node[circle,draw,fill=red!40] at (-9, 4) {};
 \node[circle,draw,fill=pink!40] at (-9, 3) {};
 \node[circle,draw,fill=orange!40] at (-9.25, 3.5) {};
 \node[circle,draw,fill=blue!40] at (-7, 3) {}; 
 \node[circle,draw,fill=green!40] at (-7, 4) {};
 
 \draw[->] (-8,5) -- (-8,6) {};
 \node at (-8,6.25) {No Increased Sharing};


 % MIDDLE

 \node[bob,minimum size=1cm] at (-2,.5) {};
 \node at (2,.5) {Description: \emph{Risk}};
 
 \node at (-2,-.5) {User Concerns:};
 \node[circle,draw,fill=blue!40] at (-1.75, -1) {};
 \node[circle,draw,fill=yellow!40] at (-2.25, -1) {};

 \node at (2,-.5) {Description Effects:};
 \node[circle,draw,fill=red!40] at (1, -1) {};
 \node[circle,draw,fill=orange!40] at (1.5, -1) {};
 \node[circle,draw,fill=green!40] at (2, -1) {};
 \node[circle,draw,fill=blue!40] at (2.5, -1) {};
 \node[circle,draw,fill=pink!40] at (3, -1) {};
 
 \draw [->] (-2,1.25) -- (-1,2.125);
 
 \draw [->] (2,1.25) -- (1,2.125);
 
 \node[circle,draw,minimum size=70] at (-.5, 3.5) {};
 \node[circle,draw,minimum size=70] at (.5, 3.5) {};
 \node at (0,1.75) {Partial Overlap};
 
 \node[circle,draw,fill=blue!40] at (0, 3.5) {};
 \node[circle,draw,fill=yellow!40] at (-1.25, 3.5) {};
 \node[circle,draw,fill=red!40] at (1, 4.25) {};
 \node[circle,draw,fill=orange!40] at (1.25, 3.75) {};
 \node[circle,draw,fill=green!40] at (1.25, 3.25) {};
 \node[circle,draw,fill=pink!40] at (1, 2.75) {};

 \draw[->] (0,5) -- (0,6) {};
 \node at (0,6.25) {Some Increased Sharing};
 
% Right
 
 \node[charlie,minimum size=1cm] at (6,.5) {};
 \node at (10,.5) {Description: \emph{Techniques}};
 
 \node at (6,-.5) {User Concerns:};
 \node[circle,draw,fill=green!40] at (5.5, -1) {};
 \node[circle,draw,fill=blue!40] at (6, -1) {};
 \node[circle,draw,fill=pink!40] at (6.5, -1) {};

 \node at (10,-.5) {Description Effects:};
 \node[circle,draw,fill=green!40] at (9.5, -1) {};
 \node[circle,draw,fill=blue!40] at (10, -1) {};
 \node[circle,draw,fill=pink!40] at (10.5, -1) {};
 
 
 \draw [->] (6,1.25) -- (7,2.125);
 
 \draw [->] (10,1.25) -- (9,2.125);
 
 \node[circle,draw,minimum size=70] at (7.5, 3.5) {};
 \node[circle,draw,minimum size=70] at (8.5, 3.5) {};
 \node at (8,1.75) {Full Overlap};
 
 \draw[->] (8,5) -- (8,6) {};
 \node at (8,6.25) {Significantly Increased Sharing};

 \node[circle,draw,fill=green!40] at (8, 4) {};
 \node[circle,draw,fill=blue!40] at (8, 3.5) {};
 \node[circle,draw,fill=pink!40] at (8, 3) {};


		\end{tikzpicture}
	}
	\caption{Visualization of our framework for reasoning about the impact of DP descriptions on users willingness to share information. Colored dots under users represent information flows about which that user cares. Colored dots under descriptions represent the information flows for which the description raises expectations. We imagine a potential user with some prior set of information disclosures about which they are concerned. When asked if they are willing to share their information with a differentially private system, the user is given a brief description of DP. Our results suggest that user's willingness to share information is not simply a function of how this description raises their expectations, but also a function of their prior concerns. Specifically, the description may raise the user's expectations for information disclosures about which the user was not concerned. Thus, we speculate, that the degree to which the user's expectations overlap with the effects of a description will be an important determining factor in a user's willingness to share.}
	\label{fig:framework}
\end{figure*}

\section{Results and Discussions}\label{sec:discussion}
Due to space constraints, we are unable to include our analysis techniques, graphs, and regression tables in this abstract.  They can be found in the full version of our work.  Below, we describe an overview of our results in text form.

\smallskip \noindent
\textbf{(RQ1) What Information Disclosures Concern Users?} We find that the most respondents --- 60.3\% --- care about information disclosures to third-parties (Share). Over half (55.3\%) care about disclosures to the person or organization running the initiative to which they contributed their information, while 52.1\% care about disclosure of their information to an entity that hacks the organization to which they contributed their information. Fewer, 43.5\%, care about whether a data analyst working at the organization might be able to learn their private information or whether graphs created using their information might disclose their private information (40.8\%). Finally, 39.8\% of respondents care whether law enforcement might be able to access their information using a court order.

\smallskip \noindent
\textbf{(RQ2) How Does the Probability of Information Disclosure Influence Sharing?} Our analysis shows that explicitly setting respondents expectations about the risk of information disclosure to certain entities does impact their willingness to share their data.  Namely, respondents were more likely to share their information\footnote{Relative to when there was a high risk of information disclosure.  Measured among the respondents who indicated they cared about the specific information disclose.} if there was no risk of information disclosure to hackers, law enforcement, organizational entities, and sharing of the data could not happen. Additionally, we find that reducing the probability of information disclosure to hackers and organizational entities from high risk to low risk also increased respondents willingness to share.  We include a more complete representation of these results in the full version of our work.

\smallskip \noindent
\textbf{(RQ3) How Do Differential Privacy Descriptions Affect Privacy Expectations?} We find that most of the different descriptions of differential privacy derived from in-the-wild descriptions do, in fact, impact user's privacy expectations.  However, descriptions changed respondents privacy expectations differently.  For example, we found that most of the descriptions raised respondent's privacy expectations against hackers, data analysts, and information disclosure through graphs or informational charts. However, only the descriptions that focused on the reduced risk associated with sharing data raised privacy expectations against information disclosures to law enforcement.  The descriptions that focused on the techniques of DP, the reduced risk to the user associated with DP, and the highly technical description all increase privacy expectations with respect to data sharing.

We also compared users expectations to the ground truth of the privacy provided by a ``typical'' differential privacy deployment, both in the local and central models. This is important as our goal is to \emph{correctly} set user privacy expectations, not simply raise them.  We find that respondents' expectations of differential privacy are more in line with the guarantees provided with the central model than the local model (that is, they have lower privacy expectations).  However, we note that user's expectations are poorly aligned with both the local and central DP models, indicating that users do not have a coherent mental model of the data collection process, as many of the privacy expectations about which we ask are equivalent from a technical perspective.

\smallskip \noindent
\textbf{(RQ4)  How Do In-The-Wild Descriptions of Differential Privacy Affect Sharing?} We find that respondents told that their information would be protected by DP --- as described by one of our descriptions --- were not significantly more willing to share their data.  This was true across all of our descriptions.


\smallskip \noindent
\textbf{Summary of Findings.} Our surveys indicate that (RQ1) users care about the kind of information disclosures against which DP can protect, and (RQ2) users' willingness to share information is significantly related to the degree of risk of most information disclosures occurring. However, the risk of disclosures occurring through the two information flows that might seem most appropriate~\cite{nissenbaum2004privacy} to users given our scenarios related to a salary transparency initiative and a medical research initiative --- disclosures through graphs or to a data analyst --- did not significantly relate to users' willingness to share. This is noteworthy, as ensuring privacy in graphs and informational charts is a common motivating example of DP, is the only information disclosure protected against by both local and central DP, and at least one current deployment of DP is focused on protecting user information from data analysts \cite{uberdpconference}.

We also find that in-the-wild descriptions of DP have a substantial impact on user privacy expectations (RQ3), but not user willingness to share (RQ4). Descriptions of DP that focus on different themes raise privacy expectations for information flows. However, we find that this can be a double-edged sword, as raising expectations can also mislead users about the system's properties.

\smallskip \noindent
\textbf{Novel framework for reasoning about the impact of descriptions.} Upon first inspection, there appears to be a contradiction embedded in our results. Namely, we established that respondents care about information disclosures relevant to DP and are (in some cases) more willing to share their information when they are assured that these information disclosures will not occur. But, we found that offering respondents DP did \emph{not} increase their willingness to share information, no matter the description. At first glance, these results might seem to indicate that respondents did not understand the descriptions at all. However, our results show that respondents had higher privacy expectations when presented with some descriptions. One would expect that these higher expectations would lead to higher willingness to share, in-line with our first results.

To resolve this tension, we recall that not every respondent cared about every kind of information disclosure. While many respondents cared about each kind of disclosure, none of the information disclosures were important to more than 60\% of respondents. Thus, there was almost certainly misalignment between the disclosures that mattered to a given respondent and the disclosures that were influenced by the DP description they were shown. For instance, imagine a potential user cared about the \emph{share} expectation, but was presented with the \emph{Trust} description. This potential user's higher expectations for \emph{hack} and \emph{data analyst} disclosures would likely do little to raise their willingness to share.

These results suggest a framework for understanding how descriptions of DP influence a user's willingness to share information (visualized in \cref{fig:framework}). When users encounter a differentially private system, they already have privacy preferences and concerns. When a user sees a description of DP, the user's expectations about certain information flows may increase. If the ways in which their privacy expectations increase aligns with the types of information disclosure about which they are concerned, they may be more likely to share their private information.  A key takeaway from this framework is that a clear and concise description of DP may not be enough to raise user's willingness to share. Instead, it is important that a description speaks to user's concerns directly and be tailored to address those concerns. 
%
% \elissa{this next part could move to discussion; I put it in intro for now but a paraphrased version probably goes in discussion} Thus, while (1) respondents do care about the data leaks against which DP can protect; (2) the likelihood of those leaks influences respondents' willingness to share; and (3) different in-the-wild descriptions of DP influence respondents perception of the likelihood of those leaks -- and the correctness of their perceptions, simply being shown a randomly-selected, in-the-wild description of DP does not increase willingness to share. We hypothesize that this is the case because each respondent only cares about certain data leaks, and each description only effects certain data leak likelihood perceptions. Thus, the probability that a given respondent was (a) shown a description that related to the data leaks they care about and (b) that description influenced enough of their perceptions is likely low. In the next section we discuss potential next steps and approaches to mitigating this issue.

% \smallskip \noindent
% \textbf{Need for new descriptions.} It is very evident from our results that the way DP is described in the wild is insufficient to help users make informed decisions. There is no consistency or standardization in the language organizations use. Thus, characterizing the way users might see DP described required us to identify the six descriptive themes used in this work. The themes present in these descriptions seem to haphazardly raise users' expectations. This is especially concerning given the differences between local and central DP; if descriptions are not carefully tailored to the model, they may mislead users about the privacy properties of the system. Indeed, \cref{fig:distributions} clearly shows that the existing descriptions of DP do little to correctly set expectations, no matter the deployment model.

% We note that the simple descriptions that we showed respondents in our surveys are not completely ineffective or without use. For instance, using our \emph{Risk} description may be appropriate for a local DP deployment as it raised expectations broadly. However, because these descriptions do nothing to increase participation, they may not achieve the goals of system designers. 

% There are two main alternatives for improving the state of DP descriptions. First, one could take the approach of Xiong et al. \cite{SP:XWLJ20}, carefully constructing descriptions of DP and training users to understand those descriptions. However, Xiong et. al.'s results indicate that such an approach is difficult: a significant number of users were unable to correctly answer test questions about DP after viewing carefully crafted descriptions. An alternative approach, which prior work on privacy beyond DP suggests may be particularly effective~\cite{schaub2017designing}, is to explicitly inform users about the risks posed to their information. For instance, a description of a central DP system might specify that information will not be leaked through any graphs or informational chats, but could still be leaked to the other entities listed above. This would be similar to the privacy nutrition labels proposed by Kelley et al. \cite{kelley2009nutrition}. Such descriptions of DP could allow users to make an informed information sharing decision without requiring them to build a comprehensive mental model of the technical details of DP techniques. That said, technical details and parameter choices for DP deployment (e.g., the value of $\epsilon$) have important implications for user privacy and, as such, future work should also explore how best to communicate these technical nuances in meaningful ways.


